Parallel Strong Connectivity Based on Faster Reachability

Computing strongly connected components (SCC) is a fundamental problems in graph processing. As today's real-world graphs are getting larger and larger, parallel SCC is increasingly important. SCC is challenging in the parallel setting and is particularly hard on large-diameter graphs. Many existing parallel SCC implementations can be even slower than Tarjan's sequential algorithm on large-diameter graphs. To tackle this challenge, we propose an efficient parallel SCC implementation using a new parallel reachability algorithm. Our solution is based on a novel idea referred to as vertical granularity control (VGC). It breaks the synchronization barriers to increase parallelism and hide scheduling overhead. To use VGC in our SCC algorithm, we also design an efficient data structure called the \emph{parallel hash bag}. It uses parallel dynamic resizing to avoid redundant work in maintaining frontiers (vertices processed in a round). We implement the parallel SCC algorithm by Blelloch et al.\ (J.\ ACM, 2020) using our new parallel reachability algorithm. We compare our implementation to the state-of-the-art systems, including GBBS, iSpan, Multi-step, and our highly optimized Tarjan's (sequential) algorithm, on 18 graphs, including social, web, $k$-NN, and lattice graphs. On a machine with 96 cores, our implementation is the fastest on 16 out of 18 graphs. On average (geometric means) over all graphs, our SCC is 6.0$\times$ faster than the best previous parallel code (GBBS), 12.8$\times$ faster than Tarjan's sequential algorithms, and 2.7$\times$ faster than the \emph{best existing implementation on each graph}. We believe that our techniques are of independent interest. We also apply our parallel hash bag and VGC scheme to other graph problems, including connectivity and least-element lists (LE-lists).

==> algo-biconnectivity.tex <==
\newcommand{\nosemic}{\renewcommand{\@endalgocfline}{\relax}}% Drop semi-colon ;
\newcommand{\dosemic}{\renewcommand{\@endalgocfline}{\algocf@endline}}% Reinstate semi-colon ;
\newcommand{\popline}{\Indm\dosemic}% Undent
\newcommand{\pushline}{\Indp}% Indent

\begin{algorithm}[t]
\small
\caption{The \VL biconnectivity algorithm\label{alg:bcc}}
\KwIn{An undirected graph $G=(V,E)$}
\KwOut{The BC-labeling for $G$}
\SetKwInOut{Maintains}{Maintains}
\SetKwProg{myfunc}{Function}{}{}
\SetKwFor{parForEach}{ParallelForEach}{do}{endfor}
\Maintains{\\
\pushline %\pushline
\noindent $\first(v)$ / $\last(v)$, the ranks of the first / last appearances of vertex $v$ in Euler tour \newline
  $\low(v)$ / $\high(v)$, the smallest / largest ranks of vertices either $v$'s subtree, or adjacent to $v$'s subtree by a non-tree edge}
\DontPrintSemicolon

Compute the spanning forest $F$ of $G$ \label{line:firstcc}\Comment{First run of CC}\\
Root all trees in $F$ using the Euler tour technique \label{line:ett}\Comment{ETT}\\
Compute $\first[\cdot]$, $\last[\cdot]$, $\low[\cdot]$ and $\high[\cdot]$ of each vertex based on the Euler tour\\
Compute the vertex label $l[\cdot]$ using connectivity on $G$ with edges satisfying $\mf{Cond}(u, v)=\true$\label{line:lastcc}\Comment{Final run of CC}\\
\parForEach {$(u,v)\in E$ s.t. \mf{Critical}$(u, v)$ and $l[u]\ne l[v]$} {
  %Assign $v$'s BCC's component head as $u$\label{line:component-head}
  Set the component head of $v$'s BCC as $u$\label{line:component-head}
}
\medskip
\myfunc{\upshape \mf{Cond}$(u, v)$\label{line:bcc-cond}\Comment{Skip back and critical edges}} {
  \If{$(u, v)$ is a tree edge\label{line:bcc-tree}} {
    \Return{$\neg$ \mf{Critical}($u, v$) and $\neg$ \mf{Critical}($v, u$)}
  } \lElse {
    \Return{$\neg$ \mf{Backward}($u, v$) and $\neg$ \mf{Backward}($v, u$)}
  }
}
\myfunc{\upshape \mf{Critical}$(u, v)$} {
  \Return{$\first[u] \leq \low[v]$ and $\last[u] \geq \high[v]$\label{line:bcc-critical}}
}

\myfunc{\upshape \mf{Backward}$(u, v)$} {
  \Return{$\first[u] \leq \first[v]$ and $\last[u] \geq \first[v]$\label{line:bcc-backward}}
}

\end{algorithm}

%$first[\cdot] \gets +\infty$ \\
%$last[\cdot] \gets -\infty$ \\
%\parForEach {$i$ from $0$ to $2 \times n - 1$} {
  %$u \gets order[i]$ \\
  %\mf{WriteMin}(first[u], i) \\
  %\mf{WriteMax}(last[u], i)
%}
%$w1[\cdot] \gets first[\cdot]$ \\
%$w2[\cdot] \gets first[\cdot]$ \\
%\parForEach {$(u, v) \in V$} {
  %\If {$e(u, v)$ is a non-tree edge} {
    %$\mf{WriteMin}(w1[u], v)$ \\
    %$\mf{WriteMax}(w2[u], v)$ \\
    %$\mf{WriteMin}(w1[v], u)$ \\
    %$\mf{WriteMax}(w2[v], u)$
  %}
%}
%$st\_min \gets \mf{BuildMinSparseTable}(w1)$ \\
%$st\_max \gets \mf{BuildMaxSparseTable}(w2)$ \\
%\parForEach {$u \in V$} {
  %$low[u] \gets st\_min.\mf{Query}(first[i], last[i]+1)$ \\
  %$high[u] \gets st\_max.\mf{Query}(first[i], last[i]+1)$
%}


==> app-bcc-correctness.tex <==
\section{The Correctness of the Vertex-Labeling Algorithm}\label{sec:app-bcc}

Due to the space limit, we defer the correctness proof of our \VL algorithm for BCC here.
Throughout the analysis we assume each connected component has more than one vertex since otherwise it is a trivial case.

To start with, we will show two useful conclusions (\cref{lem:bcc-connected} and \cref{cor:art-comp-head}) for biconnected components that will be used in proving the correctness of our \VL algorithm.

\begin{lemma}\label{lem:bcc-connected}
Given a graph $G$, vertices in each BCC $C\subseteq V$ must also be connected in an arbitrary spanning forest $F$ for $G$.
\end{lemma}
\begin{proof}
  First of all, a BCC must be connected, so they can only be in one spanning tree $T$ in $F$.

  Assume to the contrary that $C$ has at least two disconnected components (each is connected) in $T$, and let the shallowest nodes (closest to the root) for both components as $u$ and $v$.
  There are two possible positions for $u$ and $v$ in the spanning tree $T$.
  The first case is that, neither $u$ or $v$ is the ancestor of the other.
  In this case, based on our assumption, there exists at least one path from $u$ to $v$ using vertices in $C$, but not any vertices on the tree path from $u$ to $v$.
  We show that the nodes on the tree path from $u$ to $v$ is also biconnected to $u$.
  Let $w$ be the parent of $u$ and on the tree path from $u$ to $v$. %(swap $u$ and $v$ if $u$ is $v$'s ancestor).
  We now show that there are two disjoint paths that connects $w$ and $v$: the tree path between $w$ and $v$ that uses no intermediate nodes from $C$, and the path from $w$ to $u$ then to $v$, only using intermediate nodes from $C$.
  Hence, $w$ and $v$ are biconnected and $w\in C$, which leads to a contradiction that $u$ and $v$ are the closest nodes to the root in this BCC.

  The second case can be proved similarly.
  WLOG assume $u$ is $v$'s ancestor, then we look at $v$'s parent $w$, and we can show that there are at least two paths from $w$ to the nearest vertex in $u$'s component, one using the tree path while the other using vertices in $C$.
  Hence, $w$ and $u$ are biconnected, which leads to a contradiction.
\end{proof}
Since each BCC must be a connected component in one spanning tree in $F$, in the BC-labeling, the unique shallowest vertex (closest to the spanning tree root) is the component head, and the rest of the vertices all have the same label for this BCC.
Using a similar argument in the proof, we can show that:
\begin{corollary}\label{cor:art-comp-head}
Each non-root component head is an articulation point.
\end{corollary}
This is because each connected component $C$ has at least two vertices, so removing the component head $h$ disconnects $h$'s parent and $h$'s child in $C$.
If not, then there are two disjoint paths between these two nodes, so $h$'s parent is also in $C$, leading to a contradiction.

Since each BCC is connected for any spanning tree, we now define a useful concept: the \emph{subset tree}.
For a given BCC $C\subseteq V$, for a vertex $u \in C$, $u$'s subset tree $S_u$ is the intersection of $u$'s subtree and the set $C$.
Due to \cref{lem:bcc-connected}, the subset trees are connected.

Next, we show that every BCC can be found by \cref{alg:bcc}.

\begin{lemma}\label{lem:correctness-algo-to-bcc}
For each BCC $C\subseteq V$, \cref{alg:bcc} assigns them to the same biconnected component.
\end{lemma}
Directly proving \cref{lem:correctness-algo-to-bcc} is highly non-trivial, so we first show an useful lemma that \cref{alg:bcc} can correctly find the component heads.

%\begin{lemma}
%Each non-root component head identified by \cref{alg:bcc} is an articulation point.
%\end{lemma}
\begin{lemma}\label{lem:proof-comp-head}
Each component head can be identified by \cref{alg:bcc} correctly.
\end{lemma}
\begin{proof}
The component heads are the shallowest vertices in the BCCs, and the non-root ones are articulation points (\cref{cor:art-comp-head}).
% shows that all non-root component heads
Now let's consider a BCC and the shallowest vertex $h\in C$, and we show that \cref{alg:bcc} can identify it.
If $h$ not the root of the spanning tree, we know that removing $h$ cuts $C\setminus \{h\}$ from the $h$'s parent, so all edges that have endpoints in $C\setminus \{h\}$ do not have other endpoints outside $h$'s subtree.
Hence, for each of $h$'s children in $C$ (assume it is $c$), we know $\first[h]\le\low[c]$ and $\high[c]\le\last[h]$, so $(c,h)$ is a critical edge.
This means $h$ is not connected to any of $h$'s children in $C$ on \cref{line:lastcc}, so $l[h]\ne l[c]$, and $h$ will be assigned as the component head of $C$.
Later in the proof of \cref{lem:correctness-algo-to-bcc}, we will show the other direction---no two heads will be assigned to one BCC $C$.

Alternatively, if $h$ is the root of the spanning tree, then based on the definition, we directly have $\first[h]\le\low[c]$ and $\high[c]\le\last[h]$.
All $h$'s tree edges are critical, so $h$ will be on its own connected component after executing \cref{line:lastcc}, and will be assigned as the component head of $C$.
\end{proof}

With \cref{lem:proof-comp-head}, we can now prove \cref{lem:correctness-algo-to-bcc}.

\begin{figure}[t]
    \includegraphics[width=.8\columnwidth]{figures/BCC-proof.pdf}
    \caption{\small An example for different cases discussed in the proof.  Dotted arrows are critical edges.  Blue straight lines are non-critical tree edges.  Orange curve lines are cross edges.  The entire graph is biconnected, and we want to show that all non-root vertices are connected via non-critical tree edges and cross edges. \label{fig:BCC-proof}}
\end{figure}


\medskip

\begin{proof}[Proof of \cref{lem:correctness-algo-to-bcc}]
We have shown in \cref{lem:proof-comp-head} that we can find the component head $h$ for a BCC $C$ correctly.
Now we show all other vertices in $C\setminus \{h\}$ are connected using the remaining edges on \cref{line:lastcc}, so combining them proves the lemma.

We prove this by first checking all tree edges in $C\setminus \{h\}$ and showing that the two endpoints are still connected, and then all $h$'s subtrees (if more than one) are connected.


Since $C$ is biconnected, $C\setminus \{h\}$ is connected in the original graph $G$.
When running the connectivity on \cref{line:lastcc}, we skip the back edges and critical tree edges.
We now show that after removing these edges, $C'=C\setminus \{h\}$ is still connected.
Assume $h$'s children in $C$ are $c_1,\dots,c_k$.
Then either $k=1$, or the subset trees $S_{c_1},\dots,S_{c_k}$ in $C$ must be connected via cross edges, since otherwise removing $h$ disconnects them into unconnected components\footnote{Here $S_{c_i}$ cannot have back edges to $h$'s ancestors or cross edges to $h$'s ancestors' other subtrees since otherwise $h$'s parent will be biconnected to $C$.}.
%This is also true for any subset tree in $C$ that the root has multiple children in $C$.
Now we will inductively prove that all vertices in $S_{c_i}$ are connected when running the connectivity on \cref{line:lastcc}.

Let $\bar{C}$ be any subset tree rooted at $\bar{c}$.
There can be three conditions for $\bar{C}$: (1) $|\bar{C}|=1$, (2) $|\bar{C}|>1$, $\bar{c}$ has only one child $c$ in $\bar{C}$; or (3) $\bar{c}$ has at least two children.
We prove inductively: case (1) is the base case and $\bar{C}$ is trivially connected since $|\bar{C}|=1$; cases (2) and (3) are induction steps and can be applied recursively.

For case (2), the there must exist an edge $(u,v)$ such that $u\in S_c$ and $v\in C\setminus S_c$ since otherwise removing $c'$ disconnects $S_c$ and $h$.
In \cref{fig:BCC-proof}, an example is when $c'$ is node 1, $c$ is node 2, and $(u,v)$ is $(2,3)$.
Due to the existence of $(u,v)$, either $\low[c]<\first[\bar{c}]$ or $\last[\bar{c}]>\high[c]$ holds, so $(\bar{c},c)$ is a tree edge but not a critical edge, which exists when running the connectivity on \cref{line:lastcc}.
Hence, \cref{alg:bcc} put $\bar{c}$ and $c$ in the same BCC, and we can apply the same argument on $S_c$ and show all vertices are connected.

Now let's consider the most complicated one: case (3).
Again assume $\bar{c}$'s children in $C$ are $c_1,\dots,c_k$.
For a subset tree $S_{c_i}\in C$, if there exists an edge $(u,v)$ such that $u\in S_{c_i}$ and $v\in C\setminus S_c$ (can either be a back edge or a cross edge), then either $\low[c]<\first[\bar{c}]$ or $\last[\bar{c}]>\high[c]$ holds.
Some example vertices for $c$ in this case are vertices 4, 5, and 6 in \cref{fig:BCC-proof}.
In this case, $(\bar{c},c_i)$ is not a critical edge, and \cref{alg:bcc} puts them in the same BCC.
We call these subset trees as connected subset trees.
For the other subset trees (e.g., those rooted at vertices 3, 7, or 8), they are either directed connected to the connected subset trees (vertices 3 and 7), or via other unconnected subset trees (vertex 8).
For a specific unconnected subset tree $S_{c_i}$, consider a cross edge $(u,v)$ such that $u\in S_{c_i}$ and $v\in \bar{C}\setminus S_{c_i}$, and let $v$'s subset tree's root be $c_j$.
Since $v\notin S_{c_i}$, the entire tree path from $c_i$ to $u$ has no critical edges, so as the tree path from $c_j$ to $v$.
Hence $c_i$ and  are connected when running the connectivity on \cref{line:lastcc}.
In \cref{fig:BCC-proof}, an example for $c_i$ is vertex 3, and $(u,v)$ is $(3,5)$ ($\bar{c}$ is vertex 0).
The tree path from 4 to 5 only contains non-critical edges due to the existence of $(5,3)$, so vertices 3 and 4 are connected.
If $v$ is in a connected subset tree, then $c_i$ and $\bar{c}$ are connected using the tree path from $c_i$ to $u$, then the cross edge from $u$ to $v$, and the tree path from $v$ to $\bar{c}$, and none of the edges are critical edges.
In the previous example, this path is 3--5--4--0.
If all such $v$ connect to unconnected subset trees, we can show that $c_i$ connects to the other $c_j$ that $v\in S_{c_j}$.
As shown above, there always exists a path to connect every unconnected subset tree to connected ones.
Otherwise, that means there exists some subset trees (that are connected to others) with no edges going out of $\bar{c}$'s subtree.
In this case, removing $\bar{c}$ disconnects $c_i$ and $\bar{c}$'s parent), which leads to a contradiction.
Hence, \cref{alg:bcc} will connect $c_i$ to $\bar{c}$ using these cross edges and the tree paths to connect them, which contains no critical edges.
Again using vertex 8 in \cref{fig:BCC-proof} as an example, although $S_8$ does not directly connect to a connected subset tree, there must exist a path to connect 8 with 8's parent 4 via other subset trees (in this example it is 8--7--5--4) since otherwise removing 4 disconnects 8 from 4's parent, which is 0.
If no such connected subset tree 5 exists, say we remove edge $(3,5)$, then vertex 4 becomes an articulation point.
Combining all above cases, we showed that all $c_i$ are connected to $\bar{c}$.
Then we can inductively show $S_{c_i}$ is connected until we reach the base case.
\end{proof}

\begin{lemma}\label{lem:cc-to-bcc}
All vertices in each connected component computed by \cref{alg:bcc} on \cref{line:lastcc} are in a biconnected component.
\end{lemma}
\begin{proof}
  Consider two vertices $u$ and $v$ in this connected component.
  Apparently $u$ and $v$ are connected in the original graph $G$, and we now show they are also biconnected.
  Since $u$ and $v$ are connected when running the connectivity on \cref{line:lastcc}, let $P=\{u=p_0,p_1,\dots,p_{k-1},v=p_k\}$ be the path that connects $u$ and $v$ that only uses cross edges and non-critical tree edges.
  %Assume to the contrary that $u$ and $v$ are not in the same connected component.

  We now show that after removing any vertex $p_i$ that $1\le i<k$ on the path $P$, $p_{i-1}$ and $p_{i+1}$ are still connected.
  This indicates that $u$ and $v$ are biconnected.
  We prove this constructively.
  There three possible cases for the local structure.
  Case 1 is that both $p_{i-1}$ and $p_{i+1}$ are the children of $p_i$ in the spanning tree.
  Since $(p_{i-1},p_i)$ is not a critical edge, there must be an edge $(x,y)$ such that $x\in S_{p_{i-1}}$ and $y\notin S_{p_i}$.
  Similarly, for $(p_i,p_{i+1})$, there exists an edge $(x',y')$ such that $x'\in S_{p_{i+1}}$ and $y\notin S_{p_i}$.
  Hence, the without using $p_i$, $p_{i-1}$ and $p_{i+1}$ are still connected using the path that consists: the tree path from $p_{i-1}$ to $x$, then $(x,y)$, the tree path from $y$ to $y'$, $(y',x')$, and finally the tree path from $x'$ to $p_{i+1}$.
  Case 2 is that one of $p_{i-1}$ and $p_{i+1}$ is the children of $p_i$ in the spanning tree, and the other is either the parent of $p_i$ or connected to $p_i$ using a cross edge.
  WLOG, let's assume $p_{i-1}$ is the child and $p_{i+1}$ is the other vertex.
  Again, since $(p_{i-1},p_i)$ is not a critical edge, there must be an edge $(x,y)$ such that $x\in S_{p_{i-1}}$ and $y\notin S_{p_i}$.
  Meanwhile, $p_{i+1}\notin S_{p_i}$ since it is either the parent of $p_i$, or the other endpoint of a cross edge (otherwise $(p_i,p_{i+1})$ is a backward edge).
  Hence, the without using $p_i$, $p_{i-1}$ and $p_{i+1}$ are still connected using the path that consists: the tree path from $p_{i-1}$ to $x$, then $(x,y)$, the tree path from $y$ to $p_{i+1}$.
  Case 3 is that $(p_{i-1},p_i)$ is a cross edge, and either $p_{i+1}$ is $p_i$'s parent or $(p_{i+1},p_i)$ is a cross edge.
  In either case, the without using $p_i$, $p_{i-1}$ and $p_{i+1}$ are still connected using the tree path from $p_{i-1}$ to $p_i$'s parent, and the tree path from $p_i$'s parent to $p_{i+1}$ if $p_{i+1}$ is not $p_i$'s parent.

  Since removing any vertex on the path $P$ does not disconnect the path, we proved that all vertices in each connected component computed by \cref{alg:bcc} on \cref{line:lastcc} are biconnected.
\end{proof}

\cref{lem:correctness-algo-to-bcc} shows that \cref{alg:bcc} can identify every BCC, and \cref{lem:cc-to-bcc} indicates that every ouput BCC by \cref{alg:bcc} is a correct BCC.
Hence, combining them together indicates that the output for \cref{alg:bcc} is correct.
Now, we can formally prove \cref{thm:bcc}.

\medskip

\begin{proof}[Proof of \cref{thm:bcc}]
  \cref{lem:correctness-algo-to-bcc,lem:cc-to-bcc} shows that \cref{alg:bcc} computes BCCs correctly.
  Regarding the cost of \cref{alg:bcc}, \cref{line:firstcc,line:lastcc} compute two graph connectivity, and the ETT on \cref{line:ett} requires semisorting at most $2(n-1)$ key-value pairs~\cite{GSSB15}.
  The semisorting algorithm from~\cite{blelloch2020optimal} uses $O(n)$ expected work and $O(\log n)$ span \whp.
  Since computing connectivity requires visiting at least all vertices and edges, the cost for semisort is asymptotically bounded, so as the cost for other steps.
  For instance, the $\low$ and $\high$ arrays can be computed using standard range minimum queries (RMQ), which uses $O(m)$ work and $O(\log n)$ span.
\end{proof}

For our BCC implementation, we use the connectivity algorithm discussed in \cref{sec:app-cc} uses $O(m+n)$ expected work and $O(\log^3 n)$ span \whp.
Hence, our BCC is work-efficient and has polylogarithmic span.
%Many theoretical connectivity algorithms~\cite{Gazit1991,ColeKT96,HalperinZ96} has $O(m+n)$ expected work and polylogarithmic span \whp, but the complicated sampling schemes make them not practical.


\hide{
In this paper, we show a theoretically efficient \BCC{} algorithm that performs $O(n+m)$ work \xiaojun{Assuming we have semisort} in $O(?)$ span. Unlike Tarjan-Vishkin's algorithm, we do not need to construct the transformed graph. Instead, we skip a set of edges in the original graph. To achieve this, we need three key components.

\textbf{Spanning forest.} To start with, we need to know the number of spanning trees in the graph and partition all vertices on the same tree together. This part can be done by the connected component (CC) algorithm. The output spanning forest is a \defn{compressed sparse row} (CSR), where we have a permutation of vertices and an offset array indicating the range of the $i$-th tree in the vertices array.

\textbf{Euler Tour Tree.} Now we know which tree each vertex belongs to. We can construct the Euler tour tree for each tree in parallel. This is in support of computing the helper values of each vertex. Specifically, we define $\first[v]$ and $\last[v]$ as the rank of the first and last appearance of vertex $v$ in its Euler tour ordering. Also, we define the low value $\low[v]$ and high value $\high[v]$ of a vertex $v \in V$ as follows:

$\low[v]$ = $\min$\{$w_1[u]$| $u$ is in the subtree rooted at $v$\}

$\high[v]$ = $\max$\{$w_2[u]$| $u$ is in the subtree rooted at $v$\}

\noindent
where

$w_1[v]=\min\{\first [u] \cup \{\first [u'] | (u, u')$ is a non-tree edge$\}\}$

$w_2[v]=\max\{\first [u] \cup \{\first [u'] | (u, u')$ is a non-tree edge$\}\}$

To query the min and max among a subtree, we first flatten the Euler tour ordering to an array by list ranking. Then we build a sparse table~\cite{blelloch2020optimal} to process range minimum/maximum queries (RMQ).

\textbf{BC-labeling.} BC-labeling allows us to efficiently query articulation points, bridges, and the biconnected component labels in $O(n)$ space instead of saving the labels of each edge.
We define a tree edge to be a \defn{critical edge} if the parent $u$ and child $v$ have $\first[u] \leq \low[v]$ and $\last[u] \geq \high[v]$.
We also define a non-tree edge $(u, v)$ to be a \defn{backward edge} if $\first[u] \leq \first[v]$ and $\last[u] \geq \first[v]$ or vice versa.
We define an edge to be a \defn{non-essential edge} if it is either critical edge or backward edge.
Then we run the connected components on the graph skipping all non-eseential edges. The connected components algorithm returns a label for each vertex.
For each component, a \defn{component head} is the parent of its cluster in the spanning tree (the parent of the root vertex is itself).
A vertex (except for the roots) is an articulation point iff. it is the head of at least one connected component. The root of a spanning tree is an articulation point iff. it is the head of at least two connected components.
An edge $(u, v)$ is a bridge iff. $u$ is the parent of $v$ in the spanning tree and $\first[v] = \low[v]$ and $\last[v] \geq \high[v]$. \xiaojun{Assuming we don't have duplicate edges. If we do have, all duplicate edges cannot be bridge. We can use a hashtable to do this.}
Two vertices are in the same biconnected component iff. they have the same label in or one is the component head of the other.
}


\hide{

assume  $c$'s children in $C$ are $c_1,\dots,c_k$, and we will show that they are connected when running the connectivity on \cref{line:lastcc}.
Consider two of them as $c_i$ and $c_j$.
We know $c_i$ and $c_j$ are connected in the original graph $G$ via $(c_i,h,c_j)$, and at least another path that only uses vertices in $C\setminus \{h\}$ (otherwise removing $h$ disconnects $c_i$ and $c_j$).
Let $P=(c_i=v_0,v_1,\dots,v_{l-1},c_j=v_l)$ be such a pass that 1) $P$ does not have backward edges since otherwise we can replace each of them as a list of tree edges in the spanning tree, and 2) contains the minimum number of cross edges.
Now we show that all edges in $P$ remain when running the connectivity on \cref{line:lastcc}.
All cross edges in $P$  are remained.
Let $(v_{i'},\dots,v_{j'})$ be a non-empty tree path, and $v_{i'}$ and $v_{j'}$ are either the ends of the path or connect to cross edges.
WLOG assume $v_{i'}$ is deeper in the spanning tree, and in this case $v_{i'}$ cannot be the start or end of the path since $c_i$ and $c_j$ are $h$'s children and are the shallowest vertices in $C$.
This means $(v_{i'-1},v_{i'})$ is a cross edge, so



We prove this by first checking all tree edges in $C\setminus \{h\}$ and showing that the two endpoints are still connected, and then all $h$'s subtrees (if more than one) are connected.

Consider a tree edge $(u,v)$ where $u,v\in C\setminus \{h\}$ and $u$ is the deeper vertex (the child).
If $(u,v)$ is not a critical edge, then it exists when running the connectivity on \cref{line:lastcc}, so $u$ and $v$ are connected.
If $(u,v)$ is a critical edge, we know there exist no edge $(x,y)~|~x\in S_u,y\in C\setminus S_v$ (otherwise either $\first[u]<\low[v]$ or $\high[u]>\last[v]$ is true), and there exists at least one edge $(x,y)~|~x\in S_u,y\in S_v\setminus S_u$.
Otherwise, if all other endpoints $y\in S_u$, then removing $v$ disconnects $S_u$ and $h$, leading to a contradiction that $S_u$ are $h$ biconnected.
Since $x$ and $y$ are in $v$'s different subtrees,
In this case, the path $P$ that contains the tree path from $u$ to $x$, then

First, we show backward edges do not affect the connectivity.
Consider a backward edge $(u,v)$ and $u$ is the deeper vertex.




For each BCC $C$, one of the three following conditions must be true: (1) $|C|=2$ and the other vertex $c$ is $h$'s child, (2) $|C|>2$, $h$ has only one child $c$ in $C$, and there exists a backward edge $(u,h)$ where $h\in C\setminus \{h,c\}$ (otherwise cutting $c$ disconnects $C$); or (3) $h$ has at least two children, and each of them has at least one edge from its subtree to its sibling's subtree (otherwise cutting it disconnects $C$).
For case (1), $\left|C\setminus \{h\}\right|=1$ so it is trivially connected.

For case (2), we show that $c$ is connected to $c$'s child $c'\in C$, and we can recursively apply the same argument for $C\setminus \{h,c\}$.
since the existence of $(u,h)$, we have  $\low[c']<\first[c]$ and $\last[c']>\high[c]$, which means $(c,c')$ is a tree edge but not a critical edge, which exists when running the connectivity on \cref{line:lastcc}.
Hence, \cref{alg:bcc} put $c$ and $c'$ in the same BCC, and we can apply the same argument and indicate that $C\setminus \{h,c\}$ are also in the same BCC.

Now let's consider the most complicated one: case (3).
Assume $h$'s children in $C$ are $c_1,\dots,c_k$.
First of all, $S_{c_1},\dots,S_{c_k}$ must be connected via cross edges, since otherwise removing $h$ disconnects them into unconnected components.
Secondly, at least

consider $h$'s children in $C$.
At least one of them, denoted as $c$, has $\low[c]<\first[c]$ or $\high[c]>\last[c]$, since there exists at least one edge from $c$'s subtree to a vertex in $C$ but not $c$'s subtree, .
Hence, $(c,h)$ is a critical edge, and $h$ will be assigned as the component head to $c$'s BCC.




Since $C$ is biconnected, $C\setminus \{h\}$ is connected in the original graph $G$.
When running the connectivity on \cref{line:lastcc}, we skip the backward edges and the tree edges that are critical.
We now show that after removing these edges, $C'=C\setminus \{h\}$ is still connected.
There can be three conditions for $C'$: (1) $|C'|=1$ and the other vertex $c$ is $h$'s child, (2) $|C'|>1$, $h$ has only one child $c$ in $C'$; or (3) $h$ has at least two children.
We prove inductively: case (1) is the base case and $C'$ is trivially connected since $|C'|=1$; cases (2) and (3) are induction steps and can be applied recursively.

For case (2), the there must exist an edge $(u,v)~|~u\in S_c,v\in C\setminus S_c$ since otherwise removing $c$ disconnects $S_c\subset\{c\}$ and $h$.
we show that $c$ is connected to $c$'s child $c'\in C$, and we can recursively apply the same argument for $C\setminus \{h,c\}$.
since the existence of $(u,h)$, we have  $\low[c']<\first[c]$ and $\last[c']>\high[c]$, which means $(c,c')$ is a tree edge but not a critical edge, which exists when running the connectivity on \cref{line:lastcc}.
Hence, \cref{alg:bcc} put $c$ and $c'$ in the same BCC, and we can apply the same argument and indicate that $C\setminus \{h,c\}$ are also in the same BCC.

Now let's consider the most complicated one: case (3).
Assume $h$'s children in $C$ are $c_1,\dots,c_k$.
First of all, $S_{c_1},\dots,S_{c_k}$ must be connected via cross edges, since otherwise removing $h$ disconnects them into unconnected components.
Secondly, at least

consider $h$'s children in $C$.
At least one of them, denoted as $c$, has $\low[c]<\first[c]$ or $\high[c]>\last[c]$, since there exists at least one edge from $c$'s subtree to a vertex in $C$ but not $c$'s subtree, .
Hence, $(c,h)$ is a critical edge, and $h$ will be assigned as the component head to $c$'s BCC.




\begin{lemma}
On \cref{line:component-head}, each BCC will be assigned a unique component head.
\end{lemma}


\begin{lemma}
On \cref{line:component-head}, each BCC will be assigned a unique component head.
\end{lemma}
\begin{proof}
  We first show that each BCC $C\subseteq V$ will not be assigned for more than one component head.
  Assume to the contrary that two vertices $u,v\in C$ are both the children of critical edges (the lower ones), and their parents $p_u$ and $p_v$ are different.
  Since $(u,p_u)$ and $(v,p_v)$ are critical edges that are filtered out in \cref{line:lastcc},
\end{proof}

}


==> bcc.tex <==
\subsection{Biconnected Components}\label{sec:bcc}
\myparagraph{Background.} Given an undirected graph $G=(V,E)$, a \defn{biconnected component} (\BCC{}) is a maximal subset $C\subseteq V$ such that $C$ is connected and remains connected after removing any vertex $v\in C$. We start with some important definitions of BCC.
An \defn{articulation point} is a vertex such that removing it increases the number of connected components.
A \defn{bridge} is an edge such that removing it increases the number of connected components.
Given a connected graph $G$, a spanning tree $T$ of $G$ is a subgraph that is a tree spanning all of the vertices of $G$ (spanning forest if $G$ is unconnected).
For simplicity in description, we assume $G$ is connected in this section, but our algorithm and implementation work on any graph.
Given a graph $G$ and a spanning tree \newchange{$T\subseteq E$}, %$T=(V,E_{T})$ rooted at $r$, %, let $d(v)$ be the depth of $v$ in $T$ (distance to the root).
an edge is a \defn{tree edge} if it is in $T$, and a \defn{non-tree} edge otherwise.
A non-tree edge is a \defn{back edge} if one endpoint is the ancestor the other endpoint, and a \defn{cross edge} otherwise.
An illustration is given in \cref{fig:algo}(b).
If $T$ is a BFS tree, there are no back edges; if $T$ is a DFS tree, there are no cross edges.

Sequentially, Hopcroft-Tarjan algorithm~\cite{hopcroft1973algorithm} finds all \BCC{}s in $O(m+n)$ work using a DFS tree.
The idea of Hopcroft-Tarjan algorithm is to identify the back edges % (no cross edges based on DFS trees)
using the label $\low[v]$ for $v\in V$:
$$\low[v] = \min\{w_1[u]~|~u\in V \text{ is in the subtree rooted at }v\}$$
where $w_1[v]=\min\{\first[u] \cup \{\first [u']~|~(u, u')\text{ is a non-tree edge}\}\}$, and $\first[u]$ is the preorder of $u\in V$ based on the DFS tree.
The BCCs can be computed once $\first[u]$ and $\low[u]$ are known.

However, DFS is generally considered to be hard to parallelize~\cite{reif1985depth}.
To achieve parallelism in BCC, Tarjan-Vishkin algorithm~\cite{tarjan1985efficient}
uses a spanning tree $T$ generated by \emph{any} connectivity algorithm.
They then root the tree $T$ using the \emph{Euler tour technique} (ETT)~\cite{tarjan1985efficient}, which also gives $T$'s preorder and postorder.
Accordingly, Tarjan-Vishkin needs to identify and deal with both the back edges and the cross edges.
In this case, in addition to $\low[\cdot]$, it also compute $\high[\cdot]$ as:
$$\high[v] = \max\{w_2[u]~|~u\in V \text{ is in the subtree rooted at }v\}$$
where $w_2[v]=\max\{\first[u] \cup \{\first [u']~|~(u, u')\text{ is a non-tree edge}\}\}$.
Then we can identify back edges and cross edges using $\low[\cdot]$ and $\high[\cdot]$, as well as the preorder of $T$ ($\first[\cdot]$) and the postorder of $T$ ($\last[\cdot]$), which all can be obtained by the Euler tour.
%Although Tarjan-Vishkin does not explicitly compute DFS ordering,
%they use $\first[u]$ as the rank of the first appearance of $u$ in the Euler tour, which has an equivalent ordering to DFS ordering.
Tarjan-Vishkin then computes the BCC of the input graph $G$ by computing the connectivity of another graph $G'=(V',E')$ where $V'=E\setminus T$, %\xiaojun{unclear},
%and each edge in $E'$ is an edge from $E$, depending on whether it is tree edge, back edge, or cross edge.
and $E'$ can be computed based on identifying tree edges, back edges, and cross edges in $E$.
Tarjan-Vishkin costs $O(m+n)$ work and polylogarithmic span. %Generating $G'$ uses $O(m+n)$ work and $O(\log n)$ span.
We refer the readers to~\cite{tarjan1985efficient} for more details about the Euler tour technique and Tarjan-Vishkin algorithm.

Tarjan-Vishkin algorithm is theoretically-efficient.
However, we are unaware of any existing publicly-available implementation of it, mainly due to the space-inefficiency in processing the new graph $G'$.
Although running connectivity requires space proportional to the number of vertices,
the number of vertices in $G'$ is $|E|$, which is the number of edges in $G$.
For instance, using the connectivity algorithm in \cref{sec:app-cc},
the space overhead is at least 40 bytes per vertex in $G'$ (i.e., per edge in $G$).
Considering the number of edges in real-world graphs (up to tens of billions, see \cref{tab:graph}),
%For real-world large-scale graphs with 64-bit edge ids, running connectivity on $G'$
%requires 40 bytes per vertex in $G'$ (i.e., per edge in $G$).
this can greatly increase memory footprint and even make $G'$ too large to fit in memory.
%For large-scale graphs~ with more than $2^{32}$ edges, generating $G'$ and computing connectivity on $G'$ requires at least 40 bytes per edge in $G$.
%In comparison, directly running connectivity on $G$ only require $O(n)$ extra space, where $n$ is usually millions to a few billion.
%This 10x space overhead makes Tarjan-Vishkin algorithm the less preferable implementation on the shared-memory parallel setting.
This space overhead makes Tarjan-Vishkin algorithm less suitable in the shared-memory parallel setting.

To address the space issue, many existing parallel BCC implementations use BFS trees~\cite{gbbs2021, cong2005experimental, slota2014simple} to avoid processing the graph $G'$. This also simplifies algorithm design since using BFS trees leads to no back edges.
%While these algorithms~\cite{gbbs, cong2005experimental, slota2014simple} identify the BCCs differently, the common theme is that they are space-efficient as they do not need to generate the auxiliary graph $G'$.
However, using BFS trees sacrifices the theoretical efficiency---the span bound becomes $\Omega(\textsf{diam}(G))$, so these algorithms can be slower than the sequential algorithm on large-diameter graphs (see \cref{tab:sccbcc}).
To date, we are unaware of any BCC implementations that are theoretically-efficient.

%To achieve efficiency both in time and in space
In our BCC algorithm we borrow the idea of \defn{BC-labeling} proposed by Ben-David et al.~\cite{BBFGGMS18}.
Instead of labeling all $m$ edges as in the standard BCC output, BC-labeling assigns at most $2n$ total labels to \emph{vertices}.
%BC-labeling uses at most $2n$ labels to represent the BCC information, instead of size $m$ as in standard representation~\cite{jaja92}).
In BC-labeling, each vertex $v$ other than the spanning tree root has a label indicating which BCC $v$ is in.
All vertices with the same label, plus an other vertex called the \defn{component head} attached to this label, form a BCC.
See \cref{fig:algo}(b) as an example of BC-labeling.
%In addition, each BCC also has another vertex, referred to as the component head.
%All vertices with the same label and the component head of this BCC form a BCC.
Ben-David et al. showed how to retrieve articulation points and bridges from the BC-labeling,
but they did not show how to efficiently compute the BC-labeling for a graph.
We will use BC-labeling to represent our output,
and show a new algorithm to compute the BC-labeling with correctness and cost analysis.
%We omit more details here since they are independent with the contribution of this paper, but they can be found in~\cite{BBFGGMS18}.


\hide{%old
Given an undirected graph $G=(V,E)$, a \defn{biconnected component} (\BCC{}) is a maximal subset $C\subseteq V$ such that $C$ is connected and remains connected after removing any vertex $v\in C$.
An \defn{articulation point} is a vertex such that removing it increases the number of connected components.
A \defn{bridge} is an edge such that removing it increases the number of connected components.
Sequentially, Hopcroft-Tarjan algorithm~\cite{hopcroft1973algorithm} finds all \BCC{}s in a graph by using depth-first search (DFS), with $O(m+n)$ work.
However, DFS is generally considered to be hard to parallelize~\cite{reif1985depth}.

\myparagraph{Previous Parallel BCC Algorithms}.
Tarjan-Vishkin algorithm~\cite{tarjan1985efficient} achieves $O(m+n)$ work and polylogarithmic span, based on two main techniques.
The first one is to use an \emph{arbitrary} spanning tree $T$ instead of a DFS tree.
As such, Tarjan-Vishkin algorithm can use any connectivity algorithm to generate a spanning tree, and use the \emph{Euler tour technique} (ETT) to root the tree.
\yihan{explain cross edge, forward and backward edges.}
Since cross edges can show up in an arbitrary spanning tree (DFS trees only have forward and backward edges), in addition to compute the low value for each vertex as:
$$\low[v] = \min\{w_1[u]~|~u\in V \text{ is in the subtree rooted at }v\}$$
where $w_1[v]=\min\{\first[u] \cup \{\first [u']~|~(u, u')\text{ is a non-tree edge}\}\}$, the same as the sequential Hopcroft-Tarjan algorithm~\cite{hopcroft1973algorithm}, Tarjan-Vishkin algorithm also computes:
$$\high[v] = \max\{w_2[u]~|~u\in V \text{ is in the subtree rooted at }v\}$$
where $w_2[v]=\max\{\first[u] \cup \{\first [u']~|~(u, u')\text{ is a non-tree edge}\}\}$.

The second algorithmic idea in this algorithm is that, once the $\low$ and $\high$ arrays are computed, the BCC of the input graph $G$ is reduced to the connectivity of $G'=(V',E')$ where $V'=E\setminus T$, and generating $G'$ uses $O(m+n)$ work and $O(\log n)$ span.

Tarjan-Vishkin algorithm provides a genius idea to reduce BCC to connectivity (plus $O(m+n)$ additional work).
However, we are unaware of any publicly available implementation of it, mainly due to the space-inefficiency in generating the new graph $G'$.
For large-scale graphs~\cref{tab:graph} with more than $2^{32}$ edges, generating $G'$ and computing connectivity on $G'$ requires at least 40 bytes per edge in $G$.
In comparison, directly running connectivity on $G$ only uses 4 bytes per edge, plus possible compression, assuming $n\ll m$.
This 10x space overhead makes Tarjan-Vishkin algorithm the less preferable implementation on the shared-memory parallel setting.

Unlike Tarjan-Vishkin algorithm, existing parallel BCC implementations all use BFS trees~\cite{gbbs, cong2005experimental, slota2014simple}.
The benefit of using BFS trees is to avoid dealing with backward edges.
Existing BFS-based solutions~\cite{gbbs, cong2005experimental, slota2014simple} are space-efficient as they do not to generate $G'$, but their span bounds are $\Omega(\textsf{diam}(G))$, which is not theoretically efficient and can lead to slower performance than the sequential algorithm on large-diameter graphs (see \cref{tab:sccbcc}).
To date, we are unaware of any BCC implementations that are theoretically-efficient.

Recently, BC-labeling was proposed by Ben-David et al.~\cite{BBFGGMS18}, which shows a compressed representation for the BCC's output of size at most $2n$ (originally of size $m$~\cite{jaja92}).
In this representation, each vertex $v$ other than the spanning tree root has a vertex label indicating which BCC $v$ is in.
In addition, each BCC also has another vertex, referred to as the component head.
All vertices with the same label and the component head of this BCC form a BCC.
Articulation points and bridges can be easily retrieved once we have the BC-labeling.
We also use BC-labeling to represent our output.
However, Ben-David et al.~\cite{BBFGGMS18} did not show how to efficiently compute the BC-labeling of any given graph.
%We omit more details here since they are independent with the contribution of this paper, but they can be found in~\cite{BBFGGMS18}.
}

\input{algo-biconnectivity}
\myparagraph{The Vertex-Labeling Algorithm}.
We show a new parallel BCC algorithm that is work-efficient, space-efficient, and has polylogarithmic span.
%It is in some sense similar to Tarjan-Vishkin algorithm that is based on an arbitrary spanning tree, instead of a BFS tree or a DFS tree.
Our algorithm is similar to Tarjan-Vishkin algorithm in that we only need an arbitrary spanning tree (can be acquired in polylogarithmic span),
instead of a BFS tree or a DFS tree,
but avoids the $O(m)$ space overhead to process the auxiliary graph $G'$.
Avoiding generating $G'$ also makes the algorithm very simple.
%Our algorithm also only needs an arbitrary spanning tree, instead of a BFS tree or a DFS tree.
%it does not require generating the additional graph $G$, so algorithmically the new algorithm is surprisingly simple (although good practical performance requires careful engineering).

Our algorithm is given in \cref{alg:bcc}, and an illustration is shown in \cref{fig:BCC-steps}.
The first several steps are to
generate spanning forest with a CC algorithm,
construct Euler tour,
and compute the $\first$, $\last$, $\low$, and $\high$ arrays,
as in Tarjan-Vishkin algorithm.
Then instead of generating the auxiliary graph $G'$, our key insight is that we only run connectivity on the \emph{original} graph $G$,
but skipping back edges (checked by \cref{line:bcc-backward}) and \defn{critical edges} (checked by \cref{line:bcc-critical}).
%Here a backward edge is a non-tree edge that one endpoint is the other endpoint's parent, and can be checked on \cref{line:bcc-tree,line:bcc-backward}.
%A critical edge is a tree edge that all edges in the child's subtree do not ``escape'' the parent's subtree (the other endpoints are also in the parent's subtree), and can be checked on  \cref{line:bcc-tree,line:bcc-critical}.
An edge $(u,v)$ is \emph{critical} if $u$ is the parent of $v$ in the spanning tree, and none of the vertices in $v$'s subtree is connected to another vertex outside $u$'s subtree.
%A critical edge is a tree edge $(u,v)$ where $u$ is the parent of $v$, and there does not exist edge $(v',v'')$, where $v'$ is in $v$'s subtree, but $v''$ is not in $u$'s subtree.
%parent's subtree (the other endpoints are also in the parent's subtree), and can be checked on  \cref{line:bcc-tree,line:bcc-critical}.
Lastly, we check all critical edges, %and assign the child's BCC's component head as the parent.
and set the component head of the child's BCC as the parent.
We call this algorithm the \VL{} algorithm since we assign labels to the vertices (\cref{line:lastcc}), as opposed to edges in Tarjan-Vishkin algorithm.

While \cref{alg:bcc} is simple, showing the correctness is highly non-trivial. %, which might be the reason that it was previously unknown.
Given the complication of the analysis, we show the full analysis in \cref{sec:app-bcc}, and only give the theorem here.

\begin{theorem}\label{thm:bcc}
  \cref{alg:bcc} correctly computes the biconnected components of a graph $G$ with $n$ vertices and $m$ edges using $O(W_{\smb{CC}}(n,m))$ work and $O(D_{\smb{CC}}(n,m))$ span, where $W_{\smb{CC}}(n,m)$ and $D_{\smb{CC}}(n,m)$ are the work and span for graph connectivity.
\end{theorem}

%The semisorting algorithm from~\cite{blelloch2020optimal} uses $O(n)$ expected work and $O(\log n)$ span \whp.
Using the CC algorithm in \cref{sec:app-cc} gives $O(m+n)$ expected work and $O(\log^3 n)$ span \whp for \cref{alg:bcc}.
In practice, we also apply hash bags and local searches to the
two computations of connectivity (once for generating the spanning trees and another time to compute the BC-labeling).
%Hence, the work and span bounds for \cref{alg:bcc} is also decided by the graph connectivity.
%Using a connectivity algorithm that is both theoretically and practically efficient,
As shown in \cref{sec:exp:bcc}, our algorithm consistently outperforms all existing BCC implementations.
More implementation details are given in \cref{app:bcc}.











==> cover_page.tex <==

\begin{titlepage}
    \twocolumn[{%
     \centering \bf
     \LARGE Revision Summary: 
     Parallel Strong Connectivity Based on Faster Reachability \\[1.5em]
    }]

    We thank the reviewers for their constructive suggestions and comments.  In this letter, we summarize how we address the required and optional changes in the meta-review, as well as other revisions to address the individual comments from reviewers. We hope that these changes have addressed the reviewers' concerns. In this letter, we keep pointers to \revision{Sections}, \revision{Figures}, \revision{Tables}, and \revision{Algorithms} in the \emph{revised paper}, which is attached at the end of this cover letter. We have also highlighted the modified components in a different color for easy identification. Note that the label of the figures in the revision is different from that in the submission because we added new figures as suggested by the reviewers and reorganized them.


    \section*{Required Changes}
    \begin{tcolorbox}
        \textbf{1.} Improve the presentation and explain better the approach, including the hash bag and its role.
    \end{tcolorbox}
    We carefully revised \revision{\cref{sec:hashbag}}, and added descriptions about the role of \bagput{} and resizing. At the end of that section, we present the framework for reachability query using hash bags, along with new pseudocode shown in \revision{\cref{alg:BFS_hashbag}}.

    \begin{tcolorbox}
        \textbf{2.} Please explain better, maybe using a table, the parameters of your system.
    \end{tcolorbox}
     We summarize the notations used in our system in \revision{\cref{tab:notations}}. We provide the definition of the notations, as well as their default values if they are parameters.
    \begin{tcolorbox}
        \textbf{3.} Please discuss potential applications of the algorithm, if possible, and how it can be applied there.
    \end{tcolorbox}
    We discuss the applications of our two key techniques, hash bags and vertical granularity control (VGC) in \revision{\cref{sec:discussions}}. In summary, hash bags can be directly applied to other graph algorithms that need to maintain frontiers (a subset of vertices), and can potentially improve the performance of some existing implementations (e.g., \gbbs{} and Ligra) by replacing their current data structure (fix size arrays) with hashbags. The idea of VGC applies to traverse-based graph algorithms.
    The specific local search idea can be directly applied to algorithms that does not need traverse-order information.
    For algorithms that need traverse-order information, we need additional designs on top of local search. More details are discussed in \revision{\cref{sec:discussions}}.
    \section*{Optional Changes}
    \begin{tcolorbox}
        \textbf{1.}  The performance figures (Figures 7 and 8) on the 18 datasets could be reduced to a few representative ones.
    \end{tcolorbox}
We keep 12 representative graphs out of 18. The new figures are shown in \revision{\cref{fig:SCC_Total_Break}} and \revision{\cref{fig:SCC-rounds}}. We remove HL14, HH5, REC and REC' because they are similar to HL12, CH5, SQR and SQR' respectively.
% For graphs that are similar (such as HL14 and HL12), we only keep one of them. For the other similar pairs including HH5 and CH5, REC and SQR,  REC' and SQR', we remove the smaller one in each pair (HL14, HH5, REC, REC').
We also removed GL5 and GL15 because they are both similar to GL10 and follow the trend of the GL2--20 series.
If the paper is accepted, we plan to provide a full version to include the complete results on all graphs. 
%We have a \knn{} graph series: GL2, GL5, GL10, GL15 and GL20 that are generated from the same dataset but with different $k$, which are used to show the trends there are for different $k$.
%In the revised paper, we remove GL5, GL15 without loss of representation.


    \begin{tcolorbox}
        \textbf{2.} It would be better for an inclusive presentation to use grayscale patterns than red-and-green color schemes.
    \end{tcolorbox}
    We carefully regenerated all the figures in the paper. Although some of the figures use color information,
    we guarantee that the difference is visible and clear when printed by a black-and-white printer.
    For the heatmap \revision{\cref{fig:heatmap}}, we drew it in red and white.
    The darker (red) the background color is, the smaller the speedup number is, and thus the worse the performance is.
    For other experiment figures (\revision{\cref{fig:scale_all,fig:scale,fig:SCC-rounds,fig:SCC_Total_Break,fig:tau}}) and illustration figures (\revision{\cref{fig:hashbag,fig:gc,fig:local,fig:reachability}}) we use different markers/texture patterns to distinguish different lines/bars, and/or use colors with different grey levels.
    %a new color map that different colors have different gray values. Besides, we assign different textures or markers to further help identify different colors.

    \begin{tcolorbox}
        \textbf{3.} Figure 9. Please include the scalability curve of \gbbs{}, if possible, for comparison.
    \end{tcolorbox}

We add a new figure \revision{\cref{fig:scale_all}} to compare the scalability curves of different algorithms (ours, \gbbs{}, \ispan{}, and \multistep{}). The y-axis is the relative running time over the Tarjan's sequential algorithm.
We added a paragraph to discuss the scalability for all SCC algorithms in \revision{\cref{sec:exp:overall}}.
%Our algorithm is the only one that achieves almost linear speedup on all the six representative graphs. For all the other algorithms,
%their performance stops increasing (dropped or flattened) with more
%than 24 threads on one or more graphs. More discussion is in \revision{\cref{sec:exp:overall}}.

    \section*{Other Modifications Based on the Reviewers' Comments}


$\bullet$ \hl{R3O3/R4O3/R1W4: Explain the choice of parameter $\tau$.}

We discuss the intuition in \revision{\cref{sec:tau}} and also experimentally study the value of $\tau$ in \revision{\cref{sec:exp:tech}}. We add experiments of testing different $\tau$ with fewer number of processors. As mentioned in rebuttal, the results are shown in \revision{\cref{fig:tau}}. The trends on fewer processors are similar to those on 192 hyperthreads and are less sensitive. That is because $\tau$ trades off between scheduling overhead and load balancing, and both affect the performance more when number of processors is large.

\noindent$\bullet$ \hl{R1W2: Evaluate hash bags and add more related work in DB conferences.}

We add a discussion about the improvement from hash bags in \revision{\cref{sec:exp:breakdown}}.
Both our algorithm and \gbbs{} use the BGSS algorithm and perform the same computation in each round if we do not use VGC.
Hence, we compare our plain version (i.e., disabling VGC) with \gbbs{} (excluding the hash table resizing time, see more details in \revision{\cref{sec:exp:breakdown}}) to evaluate the improvement from hash bags,
because the major difference between them is just the use of hash bags.

We add more citations about SCC and possible applications in database and data management.
We also add the citation of the demonstration paper of \gbbs{}~\cite{dhulipala2020graph} in GRADES-NDA'20 (in SIGMOD'20).
We did not highlight all the citations because they appear in various sections.

\noindent$\bullet$ \hl{R1D3: Explain the reason for different breakdown patterns.}

We explain this at the end of the first paragraph in \revision{\cref{sec:exp:breakdown}}.

%$\bullet$ \hl{R1W2:  and evaluate hash bags.}

\end{titlepage}
\clearpage
\pagenumbering{arabic}


==> ett.tex <==
\subsection{More Implementation Details for BCC}
\label{app:bcc}
Due to the page limit, we provide the full details of our BCC algorithm and implementation here, which consists of four steps.

\myparagraph{Spanning Forest.}
Our implementation takes any graph (either connected or disconnected) as input.
Our first step is to find out all connected components, because two disconnected vertices are not in the same biconnected component.
We plugin our connectivity algorithm in this step, with an extra work on saving all edges used to form the connected components.
These edges recover a spanning forest.
Then we partition all vertices on the same tree and their neighbors into contiguous arrays using the compressed sparse row (CSR) format.

For simplicity, we will describe our algorithm on a spanning tree instead of a spanning forest in the following parts.
Once we find all trees, we process them in parallel.

\myparagraph{Euler Tour Technique.}
Given a tree $T=(V, E)$ and let $T'=(V, E')$ be the directed graph obtained from replacing each undirected edge $(u, v)$ in $E$ with two directed edge $(u, v)$ and $(v, u)$,
an \defn{Euler tour}~\cite{tarjan1985efficient} of $T'$ is a directed circuit such that it traverses each edge exactly once (See~\cref{fig:BCC-steps}(c)).
We start with replicating each undirected edge in $T$ into two directed edges and semisorting them~\cite{GSSB15}, such that edges with the same first endpoints are contiguous.
Then we can construct a circular linked list to recover the Euler circuit.
For each directed edge $(u, v)$ such that $u$ is the parent of $v$, if it is the first outgoing edge of $u$, we link it to the first outgoing edge of $v$.
Otherwise, we link it to its backward edge (i.e., $(v, u)$).
For each directed edge $(v, u)$ such that $u$ is the parent of $v$, if $v$ is the last child of $u$, we link to the backward parent edge of $u$ (i.e., $(u, p(u))$).
Otherwise, we link to the outgoing edge of $u$ that is pointing to the next child. %\xiaojun{Rephase this part.}
After we obtain the Euler circuit of the tree, we flatten the linked list to an array by list ranking~\cite{JaJa92}, and acquire the Euler tour ordering of the appearances of each vertex.

\myparagraph{Compute Auxiliary Arrays.}\label{app:bcc:compute}
Four auxiliary arrays, $\first$, $\last$, $\low$, and $\high$, are used in the BC-labeling technique.
Computing $\first$ and $\last$ is trivial, as it only needs to find out the first and last appearances of a vertex in the Euler tour ordering.
Computing $\low$ and $\high$ is similar to each other, so we only discuss how to compute $\low$ here.
Our algorithm first initializes $w_1[v]$ (defined in \cref{sec:bcc}) with $\first[v]$ for each $v \in V$.
Then it traverses all non-tree edges $(u, v)$ and updates $w_1[u]$ and $w_1[v]$ with the minimum of $\first[u]$ and $\first[v]$.
We build a parallel sparse table~\cite{blelloch2020optimal} on $w_1$ to support range minimum queries.
Note that $\first[v]$ and $\last[v]$ reflect the range of $v$'s subtree in the Euler tour ordering.
Thus, $\low[v]$ can be computed by finding the minimum element in the $w_1$ array in the range between $\first[v]$ and $\last[v]]$. We can compute $\high$ in the same way by only replacing minimums with maximums.

\myparagraph{Last Connectivity.}
With the auxiliary arrays, we can now identify critical edges and backward edges.
Hence, we run another connectivity and skip these edges.
The connected components give the vertex labels (BC-labeling).
Finally, we loop over all critical edges and find the component heads.
Using this information, we can find all BCCs.
In particular, all vertices with the same BC-labeling and its component head form a BCC. 

\begin{figure}[t]
    \includegraphics[width=\columnwidth]{figures/BCC.pdf}

    \caption{\small \textbf{Illustrations for our BCC algorithms in steps.} (a) Input graph. (b) An arbitrary spanning tree generated by the connectivity algorithm. (c) The Euler tour of the spanning tree. Assume we start from \nodecircle{1}, then the Euler tour ordering is {1,2,5,2,3,2,4,2,1,6,7,6,8,9,8,6,1}. (d) Different edge types of the input graph, using the spanning tree generated by Euler tour. We fix the root at \nodecircle{1}.
    The tree edges are shown in arrows.
    Gray square-dotted arrows are critical edges, which are tree edges s.t. the child's subtree has no edges going out the parent's subtree.
    Red solid arrows are non-critical tree edges.
    Orange dash lines are backward edges.
    Red round-dotted lines are cross edges. See~\cref{sec:bcc} for definitions.
    All red edges (cross edges and non-critical tree edges) will be used to run connectivity algorithm.
    Then we can get the result with BC-labeling in \cref{fig:algo}.
    \label{fig:BCC-steps}}
    %\caption{\small \textbf{Illustractions for our BCC algorithms in steps.} Given an input graph as (a), we first compute an arbitrary spanning tree on it (e.g., (b)), and compute the Euler tour on the spanning tree (e.g., (c)). An Euler tour ordering of this graph is {1,2,5,2,3,2,4,2,1,6,7,6,8,9,8,6,1}. After we compute the auxiliary arrays as described in~\cref{app:bcc:compute}, we can identify tree edges as critical edges (grey dotted arrows in (d)) and non-critical edges (red solid arrows in (d)), and identify non-tree edges as cross edges (orange double lines in (d)) and backward edges (blue dash lines in (d)). \label{fig:BCC-steps}}
\end{figure} 

==> exp-bcc.tex <==
\subsection{Experiments on Biconnectivity}
\label{sec:exp:bcc}

We now discuss our BCC performance in more detail.
%The reason that our implementation is the fastest on all instances is simple: our BCC algorithm is theoretically efficient---
We are faster than all baselines in BCC because of theoretical efficiency---work-efficiency enables competitive sequential times over Hopcroft-Tarjan sequential algorithm, and polylogarithmic span ensures good speedup for all graphs.
We first compare the \emph{sequential} running time of
\seq{}, \gbbs{} and our implementation to evaluate the work.
All three algorithms are asymptotically work-efficient. %, and thus all have reasonable good performance.
However, to enable parallelism,
our algorithm traverses all edges three times (running CC for twice and computing low/high),
and \gbbs{} needs two more traversals than us (generating rooted spanning trees using BFS and filtering edges before the last CC).
%our sequential time is about 2x slower than \seq{}
Therefore, our overall sequential time is 2x slower than \seq{}, and \gbbs{} is 4x slower.
Interestingly, on scale-free graphs, our sequential time is 1.8x \emph{faster} than \seq{}, and \gbbs{}'s sequential time is only 10\% slower. 
We believe this is because
BFS-like traversal is more cache-friendly than DFS,
and scale-free graphs take advantage of dense mode when computing the two rounds of graph connectivity, which skips many edges~\cite{Beamer12}.

To evaluate the parallelism, we compare it to the previous best parallel BCC implementation in \gbbs{}.
Our average self-speedups on both scale-free graphs and large-diameter graphs are 50x,
while the self-speedup of \gbbs's BFS-based algorithm is 9.1x on large-diameter graphs and 44x on scale-free graphs.
This makes \gbbs{} only 20\% faster than \seq{} on large-diameter graphs, while ours is 13.7x better.
Overall, our parallel running time is 11.5x faster on large-diameter graphs and 2x faster on scale-free graphs than \gbbs{}.

We compare our BCC and \gbbs{}'s running time breakdown in \cref{fig:bcc-breakdown} (a complete version is in \cref{fig:BCC_Total_Break}).
Both algorithms run in four phases: 1) find CCs; 2) generate rooted spanning trees; 3) compute low/high values; and 4) run CC again to assign labels.
As mentioned, \gbbs{} traverses the graph two more times than us:
when generating rooted spanning trees, they run BFS to get a BFS tree, while we generate spanning trees during \emph{first-CC} and just run Euler tour in the second phase;
also, they filter undesired edges in \emph{last-CC}, while we directly check and skip the undesired edges.
As a result, our algorithm is consistently faster on all graphs in these two steps (the red and orange bars).
%On scale-free graphs (first three), our main savings are in constructing the rooted spanning forest (red bars) and running the last CC (orange bars).
%When generating the spanning forest, \gbbs{} requires another BFS to generate spanning trees while we directly get the spanning forest in first-CC, and then just run Euler tour to root the trees. In last-CC, our running time is also much shorter because we directly check each edge on \cref{line:bcc-cond} in \cref{alg:bcc}. \yihan{what did they do??}
On large-diameter graphs (last three in \cref{fig:bcc-breakdown}), our BCC is significantly faster in all four phases.
For generating rooted spanning trees and computing the low/high values (the red and green bars), \gbbs has $\tilde{\Theta}(\textsf{diam}(G))$ span and does not scale well, while our approach has polylogarithmic span.
For \emph{first-CC} and \emph{last-CC} (the blue and orange bars), \gbbs uses the algorithm~\cite{SDB14} that is slower than our version with \hashbag{} and local search.%the connectivity algorithm shown in this paper.

\hide{This can also be seen in \cref{fig:bcc-breakdown}.
Our time in generating rooted spanning trees (the red bar)
We also provide the breakdown running times of our BCC and \gbbs{} in \cref{fig:bcc-breakdown}.}


\hide{
We first note that even our \emph{sequential} time is close to \seq{} (Hopcroft-Tarjan sequential algorithm) because of work-efficiency.
Our implementation is 3.7x slower on large-diameter graphs, but is 1.8x faster on scale-free graphs.
We outperform \seq{} on scale-free graphs because although our BCC algorithm traverses the graph twice (Hopcroft-Tarjan does it once),
the memory access pattern for BFS-like traversal is more cache-friendly than DFS traversal.
This benefits more for scale-free graphs where the average neighborhood sizes are larger.
Combining with parallelism, our parallel BCC is 13.7x faster than \seq{} on large-diameter graphs and 95x faster on scale-free graphs.

Comparing to the previous best parallel implementation in \gbbs{}, our good performance is mostly from better parallelism.
Our average self-speedups on both scale-free graphs and large-diameter graphs are 50x,
while the speedups for \gbbs's BFS-based algorithm are 9.1x on large-diameter graphs and 44x on scale-free graphs.
This makes \gbbs{} only 20\% faster than \seq{} on large-diameter graphs, while ours is 13.7 faster.
Our sequential running time is also better than \gbbs{} (1.9x faster on large-diameter graphs and 1.6x faster on scale-free graphs).
This is because they traverse the graph three times (first-CC, BFS to root the spanning tree, and last-CC), while we only need twice (first-CC and last-CC).
% since we do not need to generate BFS trees.
%Compared to \gbbs{}, our sequential running time is 1.9x faster on large-diameter graphs and 1.6x faster on scale-free graphs.  % since we avoid the step to generate BFS trees.
Overall, our parallel running time is 11.5x faster on large-diameter graphs and 2x faster on scale-free graphs than \gbbs{}.

We also compare the breakdown running times of our BCC and \gbbs{} in \cref{fig:bcc-breakdown}.
On scale-free graphs (first three), our main savings are in constructing the rooted spanning forest (red bars) and running the last CC (orange bars).
When generating the spanning forest, \gbbs{} requires another BFS to generate spanning trees while we directly get the spanning forest in first-CC, and then just run Euler tour to root the trees. In last-CC, our running time is also much shorter because we directly check each edge on \cref{line:bcc-cond} in \cref{alg:bcc}. \yihan{what did they do??}
On large-diameter graphs (last three in \cref{fig:bcc-breakdown}), our BCC is faster on all four steps.
For Euler tour and computing the $\low$ and $\high$ arrays, \gbbs has $\tilde{\Theta}(\textsf{diam}(G))$ span and does not scale well.
For first-CC and last-CC, \gbbs uses the connectivity algorithm from~\cite{SDB14} that is slower than our approach using \hashbag{} and local search.%the connectivity algorithm shown in this paper.
}

\hide{
On scale-free graphs (first three), we save the time from: (1) constructing the Euler tour (\gbbs{} requires another BFS to generate spanning trees while we directly work on the spanning tree generated in first-CC), and (2) explicitly generating the graph for the last-CC (we directly check each edge on \cref{line:bcc-cond} in \cref{alg:bcc}).
On large-diameter graphs (last three in \cref{fig:bcc-breakdown}), our BCC is faster on all steps.
For Euler tour and computing the $\low$ and $\high$ arrays, \gbbs has $\tilde{\Theta}(\textsf{diam}(G))$ span and does not scale well.
For first-CC and last-CC, \gbbs uses the connectivity algorithm from~\cite{SDB14} that is slower than our approach using \hashbag{} and local search.%the connectivity algorithm shown in this paper.
}


\hide{
\begin{figure}[htbp]
  %\centering
  \includegraphics[width=0.5\textwidth]{figures/BCC_breakdown.pdf}
  \caption{BCC breakdown}\label{fig:BCC_breakdown}
\end{figure}
}

\hide{We now discuss our BCC performance.
As mentioned, our implementation is the fastest on all tested instance, and on average is 6x faster
than the best of the other implementations.
On of the benefits of our algorithm is that we use \emph{any} spanning tree obtained by connectivity search,
and then use ETT which takes logarithmic span.
As such the span of the algorithm is not proportional to the diameter of the graph, and exhibit consistent good performance
on all types of graphs.
Similar to SCC, on scale-free graphs, our algorithm is faster than the baselines by 1.5-3x, and the advantage is more significant on
large-diameter graphs (2.5-20x). This is because on scale-free graphs, where diameters are small, the other implementations
based on BFS still can give a shallow spanning tree. However, when the diameter is large,
the BFS-based algorithms can be even slower than Tarjan's sequential algorithm.

} 

==> exp-scc.tex <==
%\vspace{-.05in}
%\subsection{Experiments on Strong Connectivity}\label{sec:exp-scc}
%\label{sec:exp:scc}

% \begin{figure*}[htbp]
%   %\centering
%   \vspace{-.1in}
%   \begin{minipage}[t]{0.6\textwidth}
%   \centering
%     \includegraphics[width=.85\columnwidth]{figures/scc_breakdown.pdf}
%     \caption{\small\textbf{SCC breakdown compared to \gbbs{}.} \emph{Plain} means our implementation without local-search. \emph{+LS1} means to add
%     local-search in the single-reachability search to find $\mathit{SCC}_1$.  \emph{Final} means to fully enable local search. The phases of
%     the algorithm are as introduced in \cref{sec:scc}.
%     \label{fig:SCC_breakdown}}
%   \end{minipage}\hfill
%   \begin{minipage}[t]{0.38\textwidth}
%   \includegraphics[width=\columnwidth]{figures/BCC_breakdown.pdf}
%   \caption{\small\textbf{BCC breakdown compared to \gbbs.} The phases of the algorithm are introduced in \cref{sec:exp:bcc}.
%   \label{fig:bcc-breakdown}}
%   \end{minipage}
%   \vspace{-.2in}
% \end{figure*}



\hide{We compared our implementation with \gbbs, iSpan, and Multistep. The results are shown in Table \ref{tab:sccbcc}.  From column $T_{best}/ours$, we can see that our implementation is faster than all the others on most of the graphs, except on LJ and CH5. LJ is a small social graph whose running time is short, the difference between ours and the best is only 0.004 $s$. CH5 is sparse that is hard to parallelize and parallel algorithms have overhead, so the sequential Tarjan's algorithm runs fastest on this graph.  On most KNN and Synthetic graphs, whose diameters are large, our algorithm is faster than the others by more than three times. On Social and Web graphs, whose diameters are small, our algorithm is also faster than others by around two times.  Besides, our algorithm's self-speedup is over 30x on most of the graphs and up to 76.9x on HL12. On all the graphs, our self-speedup is greater than \gbbs{}', which is around 10x on most KNN and Synthetic graphs and 20x on Social and Web graphs.}


%We now discuss our SCC performance in more details. %and explain why our implementation is the fastest on almost all instances.
%The SCC algorithm contains two single-reachability searches on the first round to find $\mathit{SCC}_1$ and the later multi-reachability searches.
%On all but one scale-free graphs, the diameters are small and $\mathit{SCC}_1$ contains more than 50\% vertices,
%and just using a parallel BFS for the single-reachability searches is reasonably good since the dense mode dominates the cost.
%Even so, using \hashbag{s} and local searches still improves the performance on scale-free graphs, and
%we are always faster than the best baseline (up to 3.16x).
%Our SCC has dominating advantages on large-diameter graphs: on average, we are 6.3x faster than \seq{},
%and 9.3x faster than any existing parallel implementations (they are all slower than \seq{}).
%Our good performance comes from better parallelism, mainly due to the local search optimization.
%Compared to \gbbs{}, the fastest previous parallel SCC, our self-speedup is 1.4--37x better (see \cref{fig:speedup}).
%%the geometric means for the self-relative speedup are 37x (ours) and 5.8x (\gbbs).
%%A better illustration for the speedup is given in \cref{fig:speedup}.
%This explains why \gbbs{} is slower than Tarjan's sequential algorithm on 8 out of 14 large-diameter graphs---the BGSS SCC algorithm has $O(m\log n)$ work compared to $O(m)$ of Tarjan's sequential algorithm, so a poor speedup does not make up the factor of $O(\log n)$ loss for the total work.
%
%To better understand the performance of our algorithm, we compare the breakdown time with \gbbs{} SCC in \cref{fig:SCC_breakdown}.
%We categorize the running time into six parts (also see \cref{sec:scc} and \cref{alg:SCC}):
%1) trimming vertices with no in- or out-degrees; 2) finding $\mathit{SCC}_1$ using two single-reachability searches; 3) all multi-reachability searches;
%4) assigning labels; 5) resizing hash tables; 6) others.
%We show the breakdown figure for all graphs in the appendix (\cref{fig:SCC_Total_Break}), and six examples in \cref{fig:SCC_breakdown}.
%We tested three versions of our algorithm: the \emph{plain} version uses parallel \hashbag{s} without local search,
%the ``\emph{+LS1}'' version enables local search in single-reachability to find the first $\mathit{SCC}_1$,
%and the ``\emph{final}'' version fully enables local search in both single and multi-reachability search.
%Even our plain version is better than \gbbs{}, due to the two reasons.
%First, using parallel \hashbag{s} saves time for many graphs (e.g., ``first-SCC'' on SQR and ``multi-search'' for HH5 and GL20)---\gbbs{} has to visit the frontiers' edges multiple times to compute the next frontier, which is not needed when using \hashbag{s}. %but such redundant work is avoided using parallel hash bags.
%Another saving is from not resizing hash tables frequently since we use a better heuristic to estimate the hash table size (see details in \cref{app:scc-details}).
%
%On top of our \emph{plain} version, local searches significantly improve the performance on large-diameter graphs.
%COS5 and SQR have a large $\mathit{SCC}_1$ (more than 90\% vertices), so \textit{+LS1} greatly reduces the runtime.
%For GL5 and SQR', the improvement is mostly from the local search in the multi-reachability searches.
%%We also give the number of rounds needed in reachability searches for GL5 in \cref{tab:sccsteps} with or without local searches,
%%and more discussions in \cref{sec:exp:tech}.
%As we will show in \cref{sec:exp:tech}, local searches reduce the number of rounds in reachability queries by 5-180x, which improves the performance.


\hide{
\begin{figure}[htbp]
%\begin{SCfigure}
%  \centering
  \begin{minipage}{.68\columnwidth}
    \includegraphics[width=\columnwidth]{figures/GL5_subrounds.pdf}
  \end{minipage}
  \begin{minipage}{.3\columnwidth}
    \caption{\small \textbf{Number of rounds in SCC reachability search with and without local search optimization.}\label{fig:GL5COS5_rounds}}
  \end{minipage}
%\end{SCfigure}
\end{figure}
}

\hide{
\begin{figure}[htbp]
  \begin{minipage}{.38\columnwidth}
    \includegraphics[width=\columnwidth]{figures/GL5_subrounds.pdf}
  \end{minipage}\hfill
  \begin{minipage}{.58\columnwidth}
    \includegraphics[width=\columnwidth]{figures/type-heat2.pdf}
  \end{minipage}
  \caption{\small \textbf{(Left) Number of rounds in SCC reachability search with and without local search optimization.}
  \textbf{(Right) Speedup of ours and \gbbs{}'s running time over the standard sequential algorithms} (Tarjan's algorithm~\cite{tarjan1972depth} for SCC, and Hopcroft-Tarjan algorithm~\cite{hopcroft1973algorithm} for BCC). For multiple graphs, we compare the geometric mean across graphs.
  \label{fig:GL5COS5_rounds}}
  \vspace{-.1in}
\end{figure}
}

\hide{
On scale-free graphs, adding local search does not make much progress since their diameters are already small.
On the large-diameter graphs, as we will discuss in \cref{sec:local}, our local queue search reduces the number of single- and multi-search rounds by 10-100x.
COS5 and SQR have a large first SCC (more than 90\% vertices), and thus \textit{+LS1} significantly reduces the time.
CH5, GL5 and SQR' have small first SCC but large diameter, so adding local search to the multi-reachability queries (comparing \textit{+ls1} with \textit{final}) improves running time.
}

% \input{total_break}

% From the figure we can see, some graphs spend much more time on the \textit{First Round}, such as SQR and TW, whose largest SCC accounts for more than $80\%$ of the $V$; some graphs spend much more time on \textit{Edge Map}, such as GL5 and SQR-S, whose SCCs' sizes are relatively uniform; and other graphs are in between.








%Note that as our algorithm uses the same framework as \gbbs{} and we also choose the same random number generator,
%Compare our \textit{plain} implementation with \gbbs{},
%our implementation gains benefits from hardly resizing the hash table.

%shows the time spent by different functions on different graphs. \textit{First Round} applies simple single-source reachability queries, and \textit{Edge Map} applies reachability queries from multi-sources.

%The overhead in \gbbs{} is mostly due to reallocate memory for their hash table in each round. This is not needed for our \hashbag{}.
%because we do not need to explicitly resize our \hashbag{}

%Interestingly, one of the overhead in \gbbs{} is the resizing time on their hash table. Because of the use of local search, we have to use a heuristic to set the hash table size (see details in \cref{sec:scc}), which avoids the resizing time.
%Even without considering this saving, our \emph{plain} version is still faster than \gbbs{}, mainly from the multi-search (comparing the green part in \gbbs{} and \emph{plain}). This saving is mainly due to \hashbag{s}, since we avoid extra work of processing the frontier multiple times.



==> fig-tau-all.tex <==
\begin{figure*}[th]
  \centering
  \includegraphics[width=\textwidth]{figures/scripts/scc_tau_all.pdf}
  \caption{\small \textbf{With 192 hyper threads, the running time on different $\tau$ ranging from 1 to $2^{16}$.}  
  \label{fig:SCC_tau_all}}
\end{figure*} 

==> figure-BFS.tex <==
\begin{figure}
  \centering
  \includegraphics[width=\columnwidth]{figures/BFS.pdf}
  \caption{\small \textbf{Parallel BFS.} \newchange{$\ff_{i}$ is the frontier in round $i$.} To generate the next frontier $\ff_{i+1}$, the algorithm first needs to visit all neighbors of $\ff_{i}$ to decide which visits are successful, which gives the size of $\ff_{i+1}$ and the \emph{offset} for each $v\in \ff_{i}$ \newchange{to add neighbors} to $\ff_{i+1}$. %\xiaojun{To work on $\ff_{i+1}$ is unclear.}
  %\letong{which gives the size of $\ff_{i+1}$ and the \emph{offset} index in $\ff_{i+1}$ for each $v\in \ff_{i}$ to start work.}
  Then the algorithm processes each $v\in \ff_{i}$ again to \newchange{write the (successfully-visited) neighbors to $\ff_{i+1}$}.
  }\label{fig:BFS}
  \vspace{-.15in}
\end{figure} 

==> figure-scc_rounds.tex <==
\begin{figure*}[th]
  \centering
  \includegraphics[width=\textwidth]{figures/scripts/subrounds.pdf}
  % \vspace{-.2in}
  \caption{\small \textbf{Number of rounds with and without local search for each batch.}
  %On \knn graphs, the average numbers of rounds can be reduced by 20--180x using local queues with size at most $2^9$.
  Each data point $(x,y)$ means that in one reachability search, $y$ rounds are needed using local search, and $x$ rounds are needed without local search.
  %The number $k$ in the title of each figure means that on that graph, using local search reduces the number of rounds in reachability searches by $k$ times on average.
  The number ``avg'' for each graph is the average number of $k=y/x$ for all data points, which means, on average, using local search reduces the number of rounds needed by a factor of $k$.
  \label{fig:SCC-rounds} }
  \vspace{-.2in}
\end{figure*} 

==> graphdetails.tex <==
% \section{More Details about the Tested Graphs}
\myparagraph{Tested Graphs.}\label{app:graphdetails}
We tested 24 graphs, including four social network graphs, four web graphs, two road graphs, eight \knn{} graphs and six synthetic graphs.
Social graphs represent users and friendship on social networks.
Web graphs represent webpages or hosts and their hyperlinks.
Road networks represents roads and their connections on maps.
$k$-NN graphs are widely used in machine learning, such as graph clustering~\cite{Maier2009,Franti2006,Lucinska2012,karypis1999chameleon}, manifold learning~\cite{Tenenbaum2000}, outlier detection~\cite{Hautamaki2004}, and proximity search~\cite{Paredes2005,Chavez2010,Sebastian2002}.
Each node is multi-dimensional data point from machine learning datasets, and has $k$ edges to its $k$-nearest neighbors (excluding itself).
For synthetic graphs, we create four lattice graphs and two chains with different lengths. %\yihan{add description for the lattice graphs.}
%each vertex $u$ has four adjacent vertices $v_1, v_2, v_3, v_4$.
All lattice graphs are based on 2D lattices of different sizes, where each row and column is circular.
In SQR and REC, we add directed edges from $u$ to each of its adjacent vertex $v$ with probability 0.5,
and from $v$ to $u$ with the same probability. We then remove duplicate edges.
In the two sparser lattice graphs (SQR' and REC'),
%we add directed edges from $u$ to each of its neighbors $v$ with probability $p=0.3$, and from $v$ to $u$ with probability $0.3$.
for each of the vertex $u$ and each of its adjacent vertex $v$, we create an edge from $u$ to $v$ with probability 0.3, and create an edge from $v$ to $u$ with probability 0.3, and create no edge with probability 0.4, then remove duplicate edges.
We choose to test lattice graphs since they simulate the input for Swendsen-Wang and other probabilistic algorithms~\cite{swendsen1987nonuniversal,edwards1988generalization,barbu2005generalizingb} for the Ising and Potts models~\cite{ising1924beitrag,potts1952some}, which is a widely used application for graph connectivity.
The full statistics of the graphs are shown in \cref{tab:graphfull}.

\input{tables/graphtable-full} 

==> intro-old.tex <==
\section{Introduction}

Computing strongly connected components (SCCs) is among the most fundamental problems in graph processing.
Given a directed graph $G=(V,E)$ and $u,v\in V$, we use $u\leadsto v$ to denote that a path exists from $u$ to $v$.
Two vertices $v,u\in V$ are \defn{strongly connected} if $u\leadsto v$ and $v\leadsto u$.
An SCC is a maximal set of vertices on the graph that are strongly connected.
The SCC problem is to compute mapping $L$ from each vertex to a unique label for its strongly connected component.
% It has extensive applications in graph matching~\cite{fan2010graph}, social network analysis~\cite{mislove2007measurement}, influence maximization problem~\cite{ohsaka2014fast} and so on.
%Based on the SCC, we can contract directed graphs into directed acyclic graphs (DAGs)
SCC has extensive applications, such as analyzing social networks~\cite{mislove2007measurement}, %contracting directed graphs into directed acyclic graphs (DAGs).
graph matching~\cite{fan2010graph}, influence maximization~\cite{ohsaka2014fast}, and topological sorting~\cite{cheng2013tf,sacharidis2009topologically}.
%\xiaojun{Rephrased.}

% model verification~\cite{hojati1993bdd}.
% \yan{fill in here.}
%if and only if they are in the same connected component (CC), biconnected component (\BCC{}), or strongly connected component (SCC).
%In the paper, we will use \defn{CC}, \defn{\BCC{}}, and \defn{SCC} to refer to the three problems, respectively.
In this paper, we denote $n=|V|$ and $m=|E|$.
For simplicity of presenting the theoretical bounds, we assume $m\ge n$, but our algorithm works for any $n$ and $m$.
%To find all SCCs in the graph, we can usually assign labels to each vertex, such that two vertices have the same label if and only if they are in the same SCC.
Sequentially, Kosaraju's algorithm~\cite{aho1983data} and Tarjan's algorithm~\cite{tarjan1972depth} find all SCCs in a graph in $O(m)$ cost.

Given the large size of today's real-world graphs, it is of great importance to seek \emph{parallel solutions} for these problems.
However, parallel SCC is an extremely challenging problem~\cite{KarpR90}.
The two above-mentioned sequential SCC algorithms~\cite{aho1983data,tarjan1972depth} both use depth-first search, which is inherently sequential~\cite{reif1985depth}.
We observe that existing parallel SCC implementations (e.g.,~\cite{hong2013fast,ji2018ispan,slota2014bfs,gbbs2021}) suffer from poor performance, especially \emph{on large-diameter graphs}.
\cref{fig:heatmap} shows the speedup of \emph{parallel SCC} implementations over the \emph{sequential algorithm} on four types of graphs: social networks, web graphs, \knn{} graphs, and
lattice graphs (see details of the graphs in \cref{sec:exp,tab:graphfull}), tested on a machine with 96 cores.
On the low-diameter graphs (social and web graphs), almost all implementations achieve reasonable speedup over the sequential algorithm.
However, on \knn{} and lattice graphs with larger diameters, \defn{none of the existing parallel implementations has a better overall performance than the sequential Tarjan's algorithm}.

\input{figure-heatmap}

In this paper, we propose an \defn{algorithm and implementation for strongly connected components (SCC) that are highly parallel},
especially addressing the challenge of achieving good parallelism on large-diameter graphs.
We focus on two goals.
First, the overhead in work (total number of operations, see \cref{sec:prelim}) should not be too much compared to the sequential computation.
Second, the overhead in parallelism (i.e., the cost of managing and synchronizing threads) should be low, ideally much lower than the computation itself.
Unfortunately, none of the existing work achieves both goals.
Most existing algorithms (\ispan{}~\cite{ji2018ispan} and \multistep{}~\cite{slota2014bfs} tested in \cref{fig:heatmap} and more in \cref{sec:related})
are specifically optimized on certain types of real-world graphs.
Hence, they do not have a good worst-case guarantee and can perform poorly on other graphs.
The theoretically-efficient BGSS algorithm for SCC~\cite{blelloch2016parallelism} has $O(m\log n)$ expected work (an $O(\log n)$ factor more than the best sequential algorithm).
The algorithm was later implemented in a graph library \gbbs{}~\cite{gbbs2021}.
While this implementation has better performance than prior work, it still suffers from poor performance on larger-diameter graphs (also see \cref{fig:heatmap}).
The BGSS algorithm uses a series of
\defn{reachability searches}, %\xiaojun{I assume they're not used by GBBS.}
which means
to find all vertices reachable from a source set $S\subseteq V$ (formally defined in \cref{sec:prelim}).
In \gbbs{}, the reachability searches are implemented by the parallel breadth-first-search (BFS), which
%From a source vertex (or a set of vertices), the parallel BFS consists of a series of rounds
%to visits vertices in the increasing order of hop distances from the sources.
visits vertices in rounds in the order of hop distances from the source(s).
On large diameter graphs, BFS needs many rounds to finish,
which causes high scheduling overhead to synchronize threads between rounds.
%We review the details of parallel BFS in \cref{sec:bfs}.
%The number of rounds in BFS is the diameter of the graph.
%On large-diameter graphs, each round only processes a few vertices,
%and there is high scheduling overhead, since global synchronization of threads is needed between rounds.
This severely limits the parallelism of this implementation.

In our work, we also use the BGSS algorithm to bound the work, and propose novel approaches to achieve much higher parallelism
on \emph{all types of graphs}. Our main observation is that, in SCC, we do not need the \emph{BFS ordering} (distance information) but only the \emph{reachability} information on whether a search can reach a vertex or not.
%Namely, for a given source vertex $u$, we only need to know the set of vertices $v$ with an arbitrary path from $u$ to $v$ (directed or undirected), but not the shortest path length (given by BFS).
%Hence, replacing BFS by reachability that gives strictly less information enables spaces for potential optimizations.
This relaxation enables effective optimizations.
%The correlation between reachability and connectivity-related problems has been raised in recent theory work~\cite{blelloch2016parallelism,schudy2008finding,fineman2019nearly}.
%In this paper, we further study two questions to make the idea highly practical.
% we need to address the following two questions to enable efficiency in practice for such problems.
%First, given that we do not need to maintain the BFS ordering, how can we design a parallel reachability algorithm?
%Second, how can we use parallel reachability to design connectivity-related algorithms?
Based on this observation, we propose two techniques:
1) the \defn{local search}, which is an optimization for reachability search to reduce the costs (number of rounds) of synchronizing threads,
and 2) the \defn{\hashbag{}}, which is a data structure to efficiently maintain the vertices processed in each round (called the \defn{frontier} of each round).
%\xiaojun{Should we cite SSSP somewhere? We use the same techniques.}\yihan{We'll mention this in the corresponding sections. }

Our first technique is the \defn{local search} optimization in reachability queries.
When processing a vertex $v$, the BFS algorithm visits all neighbors of $v$, pushing out the frontier by one hop from the source.
On large-diameter graphs, this incurs a lot of rounds to finish.
In this case, the scheduling overhead (e.g., forking and synchronizing threads between rounds) is much more costly than the
actual computation, as each thread usually only visits a small number of vertices.
Our local search aims to reduce the number of rounds, thus saving the synchronization cost.
When processing a vertex $v$, in addition to the direct neighbors of $v$, we maintain a fixed-size buffer for local search in the local (stack) memory and further search outwards until the buffer is full.
%A subset of the elements in the buffer will then be flushed to the next frontier.
%a certain condition is satisfied, e.g., stop when $q$ total vertices have been visited.
%This may not visit the vertices in the BFS order, as some of them are not visited in order of the hop distances to the source.
The vertices may not be visited in the BFS order, %as some of them are not visited in order of the hop distances to the source.
but this does not affect the reachability of the vertices.
Conceptually, we believe this optimization functions as a parallel \emph{granularity control}, such that we try to \emph{let each thread perform a reasonably large amount of work}.
It is also similar to adding shortcuts to the graph on the fly to reduce the number of rounds needed.
%Surprisingly, %we were unaware of this simple yet effective optimization previously,
This simple optimization significantly improves the performance of our algorithms (e.g., 2.3--14x on \knn{} and lattice graphs ).
We discuss more details in \cref{sec:local}.


Our second technique is a data structure, called the \defn{parallel \hashbag{}}, to maintain the vertex set being processed (the \emph{frontier}) in each round.  % efficiently by dynamic resizing.
The goal is to avoid the redundant work in processing the frontier multiple times in order to count the size of the next frontier to allocate memory.
Our parallel \hashbag{} is similar to a resizable hash table but avoids copying on resizing.
%Since bag does not support the find operation,
We maintain a multiple-level structure in exponentially growing sizes without sacrificing the cost per operation.
%This is inspired by the sequential $k$-level hash table proposed by Gu et al.~\cite{gu18algorithmic}, but here we allow $k=o(1)$.
We use atomic operations to enable concurrent insertions and a sampling scheme to support resizing,
such that we do not need to know the exact size of the next frontier.
This is also important under the local search setting, where each processed vertex can explore multiple hops of the neighborhood,
and it is hard to count the number of newly-visited vertices in each round in advance.
Our \hashbag{} is theoretically-efficient %regarding work (total operations) and span (longest dependent operations),
and fast in practice.
%Interestingly, we showed that by carefully picked parameters, we can use this data structure as a parallel hash table, which outperforms previous implementations~\cite{gbbs2021}.
%Using parallel \hashbag{}s to maintain the frontiers in SCC significantly improves the performance.
We describe the \hashbag{} in detail in \cref{sec:hashbag}. %\hashbag{}s can be applied to most edge-map based algorithms, such as CC and LE-list, which simplifies coding and improves the performance.

We believe that our proposed techniques are general and of independent interest. In addition to the SCC problem, which is our main focus, we apply the proposed techniques to two more algorithms: connected components (CC) and least-element lists (LE-lists). Using our techniques, we improve the performance of a state-of-the-art CC algorithm and present the first parallel LE-lists implementation.
We overview these problems in \cref{sec:others} and present some experimental results in \cref{sec:exp-cc-lelists}.


% Among these problems, connectivity is the simplest and has many parallel algorithms and implementations (e.g., \cite{AwerbuchS83,beamer2015gap,blelloch2012internally,gbbs2021,greiner1994comparison,ShiloachV82,shun2013ligra,SDB14,dhulipala2020connectit}).
% A recent work by Dhulipala et al.~\cite{dhulipala2020connectit} implemented over 232 parallel connectivity algorithms, many of which are highly practical.
% The problems on \BCC{} and SCC are much harder.


% We know very few existing implementations,
% and most of them are based on parallel breadth-first searches (BFS).


% As implementing parallel SCC algorithms is not trivial, we know very few existing implementations (\gbbs{}~\cite{gbbs2021}, \ispan{}~\cite{ji2018ispan} and \multistep{}~\cite{slota2014bfs}), and most of them using paralell bread-first search (BFS) for reachability queries (gbbs{}~\cite{gbbs2021} and \multistep{}~\cite{slota2014bfs}).
% \letong{need to find more related work for scc implementations.}

%\letong{find more implementations}
%On identifying strongly connected components in parallel

% -------------Add more related work citation?-------------
\hide{
However, BFS itself is hard to parallelize for arbitrary graphs, which %makes the corresponding SCC and BCC
%algorithms
results in theoretically-inefficient implementations for SCC---the span of BFS is proportional to the diameter of the graph.
For instance, as shown in \cref{fig:heatmap}, in GBBS~\cite{gbbs2021},
the BFS-based SCC algorithms achieve very good performance on low-diameter graphs (e.g., social and web graphs)
but do not perform well on larger-diameter graphs (e.g., \knn{} and lattice),
and in many cases are even slower than the standard \emph{sequential} algorithms.
The reason is that on large-diameter graphs, BFS requires more rounds and visits fewer vertices in each round, which causes insufficient parallelism in each round and significant overhead for global synchronization between rounds.
Taking the geometric means on all graphs,
\gbbs{}'s SCC on 96 cores is only 2x faster than the standard \emph{sequential algorithm} (see \cref{fig:GL5COS5_rounds}).}

% \letong{add more introduction to ispan and multi-step}

% ------------Add intro for ispan and multi-step-------------------

\hide{
%As a result, almost all existing parallel \BCC{} implementations are based on BFS.
As a result, there were no existing SCC implementations with desirable performance on all graph instances tested in this paper.



Our main observation is that, in SCC and CC problems, we do not need the \emph{BFS ordering} (distance information) but only need the \emph{reachability} information on whether a search can reach a vertex or not (formal definition given in \cref{sec:technique}).
%Namely, for a given source vertex $u$, we only need to know the set of vertices $v$ with an arbitrary path from $u$ to $v$ (directed or undirected), but not the shortest path length (given by BFS).
%Hence, replacing BFS by reachability that gives strictly less information enables spaces for potential optimizations.
This relaxation enables effective optimizations in parallel implementations.
The correlation between reachability and connectivity-related problems has been raised in recent theory work~\cite{blelloch2016parallelism,schudy2008finding,fineman2019nearly}.
In this paper, we further study two questions to make the idea highly practical.
% we need to address the following two questions to enable efficiency in practice for such problems.
First, given that we do not need to maintain the BFS ordering, how can we design a parallel reachability algorithm?
Second, how can we use parallel reachability to design connectivity-related algorithms?
%The latter is especially
% important for \BCC{}, where many state-of-the-art implementations (e.g., GBBS~\cite{gbbs2021} and SM'14~\cite{slota2014simple}) \emph{require} a BFS spanning tree. If we replace BFS with reachability, how can we redesign the algorithm to guarantee correctness?
%By relaxing this condition in BFS, we are able to employ more aggressive optimizations to accelerate reachability search. For example,
%we do not need to explore neighbors in the order of the distance from the source, as is done in BFS.
%We show that t and further benefit the algorithms for CC, BCC, and SCC algorithms.
%We propose two key techniques to address the above two issues.
%We answer these questions in this paper.
}
\hide{
%To answer the first question, we need to consider what types of reachability queries we need.
The main contribution of this paper is an efficient reachability algorithm with highly-practical optimizations.
Note that this includes both single-reachability from one source and a more complicated case of multi-reachability from a set of sources,
which is used in the parallel SCC algorithm~\cite{blelloch2016parallelism}.
Our reachability algorithm is based on the parallel round-based BFS algorithm, and we show two algorithmic improvements.



Our first technique is an efficient \emph{local search} optimization in reachability queries.
When processing a vertex $v$, the BFS algorithm visits all neighbors of $v$, pushing out the frontier by one hop from the source.
On large-diameter graphs, this incurs a lot of rounds to finish, between which global synchronization is needed.
In this case, the scheduling overhead (e.g., forking and synchronizing threads) is much more costly than the
actual computation, as each thread usually only visits a small number of vertices.
Our local search aims at reducing the number of rounds and thus saving the synchronization cost.
When processing a vertex $v$, in addition to the direct neighbors of $v$, we maintain a fixed-size buffer for local search in the local (stack) memory and further search outwards until the buffer is full.
%A subset of the elements in the buffer will then be flushed to the next frontier.
%a certain condition is satisfied, e.g., stop when $q$ total vertices have been visited.
%This may not visit the vertices in the BFS order, as some of them are not visited in order of the hop distances to the source.
This may not visit the vertices in the BFS order, %as some of them are not visited in order of the hop distances to the source.
but this does not affect the reachability of the vertices.
Conceptually, we believe this optimization functions as a parallel granularity control, such that we try to \emph{let each thread perform a reasonably large amount of work},
and is also similar to adding shortcuts to the graph on the fly to reduce the number of rounds needed.
Surprisingly, we were unaware of this simple yet effective optimization previously,
which significantly improves the performance of our algorithms (e.g., 2-7x for SCC on \knn{} graphs).
We discuss more details in \cref{sec:local}.



Second, we propose a data structure, referred to as the \emph{parallel \hashbag{}}, to maintain the vertex set being processed (the \emph{frontier}) in each round efficiently.
The goal is to avoid the overhead in counting the size of the next frontier to allocate memory, which can result in redundant work in processing the frontier multiple times.
Our parallel \hashbag{} is similar to a resizable hash table but avoids copying on resizing.
%Since bag does not support the find operation,
We maintain a multiple-level structure in exponentially growing sizes without sacrificing the cost per operation.
%This is inspired by the sequential $k$-level hash table proposed by Gu et al.~\cite{gu18algorithmic}, but here we allow $k=o(1)$.
Our design uses atomic operations to enable concurrent insertions and a carefully-designed sampling scheme to support resizing at the same time,
such that we do not need to know the exact size of the next frontier.
Our \hashbag{} is theoretically efficient regarding work (total operations) and span (longest dependent operations) and fast in practice.
%Interestingly, we showed that by carefully picked parameters, we can use this data structure as a parallel hash table, which outperforms previous implementations~\cite{gbbs2021}.
Using parallel \hashbag{}s to maintain the frontiers in SCC significantly improves the performance of these algorithms.
We describe the \hashbag{} in detail in \cref{sec:hashbag}. \hashbag{}s can be applied to most edge-map based algorithms, such as CC and LE-list, which simplifies coding and improves the performance.



To answer the second question about applying reachability algorithm to the connectivity-related problems,
we have to carefully choose or redesign the relevant algorithms to decouple the features enabled by BFS
but still guarantee the correctness and cost bound of the algorithms.
All the algorithms we propose or implement in this paper have a theoretical guarantee and are highly practical.
For SCC, we plug our reachability algorithm into the BGSS algorithm~\cite{blelloch2016parallelism}
, which is theoretically efficient (wrt.\ the number of dependent reachability searches~\cite{blelloch2020randomized}).
For connectivity, we also apply our techniques to an efficient algorithm from ConnectIt~\cite{dhulipala2020connectit} and further improve the performance.
Meanwhile, we show this algorithm is theoretically efficient (the only known theoretically efficient CC algorithm~\cite{SDB14} is not as fast in practice).
We also consider the least-element lists (LE-lists)~\cite{blelloch2016parallelism}, which is a widely-used graph building block in many applications (e.g.,~\cite{cohen2004,du2013,blelloch2017efficient,Khan2008}).
We show the first parallel implementation for LE-lists based on the BGSS LE-lists algorithm~\cite{blelloch2016parallelism} using the proposed techniques.
}

%[maybe mention CC and LE-list]

Our implementations achieve good performance on various real-world and synthetic graphs (see \cref{fig:heatmap}), including
the \emph{largest publicly available graph (HL12) with 3.6 billion vertices and 128 billion edges}.
%We show a heatmap in \cref{fig:heatmap} to compare the performance of our SCC algorithm to state-of-the-art implementations,
%including one implementation based on the standard sequential Tarjan's algorithms \cite{tarjan1972depth} (implemented by us).
Among all correct implementations, our SCC implementation achieves the best performance on almost all (17 out of 18) graphs.
%\footnote{We exclude tests with wrong answers.
%We are only slower than the sequential algorithm on a small graph with a large diameter, and none of the existing parallel implementations outperform Tarjan's algorithm. See more details in \cref{sec:exp}.
%For the two exceptions, we were slower than \ispan{} on graph LJ, but \ispan{} reports wrong answer on this graph. We were slower than Tarjan's sequential algorithm on CH5, which is a small graph with a large diameter, and none of the existing parallel implementations outperform Tarjan's algorithm. See more details in \cref{sec:exp}.
%}.
Our implementation performs particularly well on large-diameter graphs (e.g., \knn{} and lattice graphs).
%Compared to the \emph{best existing parallel implementations},
On these graphs, we are 1.8--12x faster compared to the \emph{best existing parallel implementations on each graph instance}.
On small-diameter graphs, we are also 1.15--3.6x faster than the \emph{best existing parallel implementations with correct answers}.
% \xiaojun{how can we get 1.15 if we're slower than \ispan{} on LJ.}\yihan{I added ``correct answers''}
% \letong{check the 3.6x number}
\hide{
\yan{these few sentences need to be reworded. Compared to the \emph{best existing implementations},
we are 7.5-14.1x faster on BCC on road networks,
3.1-11.5x faster in SCC and 2.6--12.4x faster in BCC on \knn{} graphs (diameter up to 1600+),
1.9-53x faster in SCC and 12--300x faster in BCC on lattice graphs (diameter up to 20000+).
On low-diameter graphs such as social and web graphs (diameter mostly within 100),
our implementation also achieves comparable or much faster (up to 3.6x faster in SCC and up to 2.7x in BCC) performance compared to state-of-the-art implementations.}
}
Our experiments show that the good performance of our implementations mainly comes from local search (using 11--260x fewer rounds than BFS on large-diameter graphs) and \hashbag{}s (saving work on all types of graphs).  We release our code %\href{https://github.com/ucrparlay/Parallel-Strong-Connectivity}{https://github.com/ucrparlay/Parallel-Strong-Connectivity}.
on GitHub~\cite{scccode}. %\url{https://github.com/ucrparlay/Parallel-Strong-Connectivity}.
We summarize our contributions as follows.
%\yihan{The list of contributions does not seem very necessary. We can remove them if we need more space.}

\begin{enumerate}[wide,topsep=0pt]%labelwidth=!, , labelindent=0pt
  \item Two general techniques (parallel \hashbag{} and local search) to optimize the performance of reachability queries.
  % \item The design and analysis of a parallel biconnectivity algorithm that is theoretically efficient in work, span, and space.
  \item Fast implementations on SCC, CC, and LE-lists using the proposed techniques.
  Our SCC algorithm greatly outperforms existing implementations.
  % For BCC, our implementation is the first publicly-available theoretically-efficient parallel implementation.
  Our LE-lists implementation is the first parallel implementation.
  \item In-depth experimental evaluation of the problems and the optimizations in this paper across multiple types of graphs.
\end{enumerate}





\hide{
\begin{figure}
  \centering
  \includegraphics[width=\columnwidth]{figures/heatmap.pdf}
  \caption{Heatmap}\label{fig:heatmap}
\end{figure}
}

\hide{

Figure \cref{fig:intro1} shows the performance of GBBS, which is one of the best existing implementations for SCC and BCC.
On large social-networks, both algorithms perform reasonably well.
However on the same size of graphs with large diameter, such as road network and KNN graphs, they requires much longer running time, and for some of them even longer than processing a much larger social network.
The problem lies in that existing algorithms for BC or SCC rely on Breadth First Search (BFS) as a core component, which itself is hard for large-diameter graphs.
State-of-the-art parallel BFS algorithm processes vertices in rounds. The $i$-th round processes all $i$-hop neighbors of the source vertex in parallel, called the current \emph{frontier}, explores their neighbor sets and puts the newly visited neighbors in the next frontier.
However, BFS itself is hard to parallelize for large diameter graphs.
%When the current frontier grows large, the algorithm usually turns on a \emph{dense mode} to
There are two major issues.
%First of all, in each round, generalizing the next frontier in parallel requires to visit the neighborhood of the current frontier at least twice
First of all, to generate the next frontier in a consecutive array, the algorithm needs to visit the neighborhood of the current frontier at least twice. The first time selects the appropriate vertices (excluding the visited ones or duplicates) and compute the offset for each selected vertices, and the second time writes (packs) the selected vertices to the corresponding slots in the next frontier. This creates extra overhead in the algorithm.
For dense graphs, BFS algorithms can use a \emph{dense mode} (see details in xx) to avoid this second-round packing, but this only pays off when the frontier is large (called the dense rounds).
Secondly, on sparse graphs, the frontier size is usually small, and the number of total rounds needed may be large.
Since parallelism is explored only within each round, synchronizations are needed between rounds.
Therefore, large number of rounds directly leads to longer running time.
Again this is not an issue for dense graphs, since their diameters are small, the number of rounds is usually a small number.

Our design is based on an observation that such data structures for maintaining frontiers usually requires fast operations of
\fname{put} and \fname{forall} (in parallel), whereas a fast look up operation is not required.
Our \hashbag{} is implemented by a pre-allocated array with sufficiently large size (usually just the number of vertices in the graph),
but only uses a small prefix of size $O(s)$, where $s$ is the current number of elements in the bag.
An element is put into the bag by scattering it to an arbitrary slot in the current array, and resizing is done by swinging the tail pointer to twice of the
current size. To decide when to resize, we carefully design a sampling scheme to estimate the current size of the bag.
By putting all vertices in the next frontier to the \hashbag{}, we can reconstruct the frontier by visiting the prefix of the bag and skipping the empty slots.
This visits at most $O(s)$ elements for a frontier of size $s$, instead of visiting the full edge list of the previous frontier.

}


%Our key idea is based on two optimizations on top of the parallel round-based BFS algorithm.
%The simple case is referred to as single-reachability, in which we compute all vertices reachable by a single vertex.
%The more complicated case is multi-reachability, and we compute all vertices reachable by each of a vertex set.
%The latter case is used in some existing algorithms such as the BGSS SCC algorithm~\cite{blelloch2016parallelism}.
%We mainly focus multi-reachability since it is harder, and consider single-reachability as a special case.
%Our parallel reachability algorithm is based on parallel BFS---keep a vertex set and explore the neighbors in a round manner, but with the following two optimizations.


%Such costs largely limit the parallelism because scheduling overhead of forking and joining threads between rounds
%is much more expensive than the actual computation, as the frontier and the neighborhood size of the frontier
%This can be undesirable --- since the frontier is small and the graph is sparse, even the full size of the frontier's neighborhood is too small
%to fully employ parallelism in a reasonable powerful machine with ~100 hyperthreads.
%Each parallel task itself is too small to hide the scheduling cost (e.g., forking and joining threads).
%It has been shown that the performance many shared-memory parallel algorithms are dominated by the global synchronization time \cite{??}.

%Such costs largely limit the parallelism because scheduling overhead of forking and joining threads between rounds
%is much more expensive than the actual computation, as the frontier and the neighborhood size of the frontier
%This can be undesirable --- since the frontier is small and the graph is sparse, even the full size of the frontier's neighborhood is too small
%to fully employ parallelism in a reasonable powerful machine with ~100 hyperthreads.
%Each parallel task itself is too small to hide the scheduling cost (e.g., forking and joining threads).
%It has been shown that the performance many shared-memory parallel algorithms are dominated by the global synchronization time \cite{??}.


\hide{
There are two major difficulties
First of all, to generate the next frontier in a consecutive array, the algorithm needs to visit the neighborhood of the current frontier at least twice. The first time selects the appropriate vertices (excluding the visited ones or duplicates) and compute the offset for each selected vertices, and the second time writes (packs) the selected vertices to the corresponding slots in the next frontier. This creates extra overhead in the algorithm.
For dense graphs, BFS algorithms can use a \emph{dense mode} (see details in xx) to avoid this second-round packing, but this only pays off when the frontier is large (called the dense rounds).
Secondly, on sparse graphs, the frontier size is usually small, and the number of total rounds needed may be large.
Since parallelism is explored only within each round, synchronizations are needed between rounds.
Therefore, large number of rounds directly leads to longer running time.
Again this is not an issue for dense graphs, since their diameters are small, the number of rounds is usually a small number.
}



%To design parallel algorithms for these problems that are both theoretically and practically efficient,


==> multi_search.tex <==
\begin{figure*}
  \centering
  \includegraphics[width=.9\textwidth]{figures/subrounds.pdf}
  \vspace{-.2in}
  \caption{\small \textbf{Number of rounds with and without local search for each batch.}
  %On \knn graphs, the average numbers of rounds can be reduced by 20--180x using local queues with size at most $2^9$.
  The number $k$ in the title of each figure means that on that graph, using local search reduces the number of rounds in reachability searches by $k$ times on average.
  \label{fig:SCC-rounds}}
\end{figure*}


==> other-details.tex <==
% \section{Other Algorithmic Details for SCC and tested graphs}\label{sec:other-details}


% \subsection{More Implementation Details for SCC}\label{app:scc-details}
We also observed that hash table resizing is an expensive component in GBBS (see \cref{sec:bgssalgo}), and thus we adopt a better heuristic for estimating the size of the hash table needed to maintain all reachable pairs.
%This is also needed if local search is enabled, 
Such estimation is necessary when local search is enabled, because we can no longer upper bound of the reachability pairs, which decides the hash table size.
In GBBS, since each round only visits one-hop neighbors, they use $\sum_{v\in \ff_{i}} |N(v)| \cdot |T(v)|$ as an upper bound for number of reachability pairs in each round, where $N(v)$ are neighbors of $v$ whose labels are the same as $v$, and $T(v)$ are the pairs containing $v$ in the hash table.
In our implementation, we calculate constant fractions for the previous frontier size and the number of remaining vertices, and take the maximum of them to estimate the hash table size.
It is based on the observation that the number of reachability pairs is usually highly correlated to these two sizes.
When the hash table is too full, we restart from a larger hash table.
In most cases, resizing is not needed. 
As shown in \cref{fig:SCC_Total_Break}, on many graphs, the resizing hash tables in GBBS is costly, and we can save this part in our implementation.
% \input{ett.tex}


==> speedup.tex <==
\begin{figure*}
  \centering
  \includegraphics[width=2\columnwidth]{figures/speedup2.pdf}
  \caption{Speedup\label{fig:speedup}}
\end{figure*} 

==> tables/_Please_add_the_following_packages_if_necessary_ <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table}[!htp]\centering
\caption{Generated by Spread-LaTeX}\label{tab: }
\scriptsize
\begin{tabular}{lrrrrrrrrr}\toprule
& &n &m &diameter &|SCC1| &largest scc/n &# SCC &Notes \\\midrule
social &LJ &4847571 &68993773 &16 &3828682 &78.98\% &971232 &soc-LiveJournal1 \\
&TW &41652231 &1468365182 &65* &33479734 &80.38\% &8044729 &Twitter \\
Web &SD &89247739 &2043203933 &17* &47965727 &53.74\% &39205039 &sd\_arc \\
&CW &978408098 &42574107469 &16* &774373029 &79.15\% &135223661 &ClueWeb \\
&HL14 &1724573718 &64422807961 &793* &320754363 &18.60\% &1290550195 &Hyperlink14 \\
&HL12 &3563602789 &128736914167 &5275* &1827543757 &51.28\% &1279696892 &Hyperlink12 \\
KNN &HH-5 &2049280 &10246400 &980* &257914 &12.59\% &94010 &Household with k=5 \\
&Ch-5 &4208261 &21041305 &4550* &497331 &11.82\% &248227 &CHEM with k=5 \\
&GL-2 &24876978 &49753956 &13* &5368 &0.02\% &9705931 &GeoLife with k=2 \\
&GL-5 &24876978 &124384890 &4622* &860403 &3.46\% &3198626 &GeoLife with k=5 \\
&GL-10 &24876978 &248769780 &3172* &3042330 &12.23\% &326811 &GeoLife with k=10 \\
&GL-15 &24876978 &373154670 &5491* &3239156 &13.02\% &187646 &GeoLife with k=15 \\
&GL-20 &24876978 &497539560 &5275* &3336963 &13.41\% &128021 &GeoLife with k=20 \\
&COS-5 &321065547 &1605327735 &1148* &301413787 &93.88\% &2273690 &COSMO50 with k=5 \\
Synthetic &SQR &100000000 &300000074 &10002* &99101606 &99.10\% &829,495 &2D grid 10^4*10^4 \\
&REC &10000000 &30000778 &5946* &9890647 &98.91\% &101059 &2D grid 10^3*10^4 \\
&SQR-S &100000000 &120299012 &14* &58 &0.00\% &78052793 &sampled 2D grid 10^4*10^4 \\
&REC-S &10000000 &12031898 &80* &42 &0.00\% &7819050 &sampled 2D grid 10^3*10^4 \\
\bottomrule
\end{tabular}
\end{table}

==> tables/bccscctable.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet3'
\newcommand{\goleft}{-.3em}
\newcommand{\cellcolorhighlight}{\cellcolor[rgb]{ 1,  1,  0.5}}
\newcommand{\textcolorhighlight}{\textcolor[rgb]{ 1,  0,  0}}
\begin{table*}[htbp]
  \centering \small

    \begin{tabular}{@{}c@{  }@{  }l|r@{  }@{  }r@{  }@{  }r|r@{  }@{  }r@{  }@{  }r|r@{  }@{  }r@{  }@{  }r|r|r@{  }@{  }r@{  }@{  }r|r@{  }@{  }r@{  }@{  }r|r@{  }r|r}
          &       & \multicolumn{10}{c|}{\textbf{SCC}}                                            & \multicolumn{9}{c}{\textbf{BCC}} \\
%\cmidrule{3-21}
          &       &
          \multicolumn{3}{c|}{\textbf{Ours}} &
          \multicolumn{3}{c|}{\textbf{GBBS}} &
          \multirow{2}{*}{\textbf{iSpan}} & \multicolumn{1}{@{}c@{}}{\textbf{Multi-}} & \multirow{2}{*}{\textbf{ \seq{}}} & %@{}c@{}|
          \multicolumn{1}{c|}{\cellcolorhighlight\boldmath{}\textbf{$\boldsymbol{T_{\mathit{best}}}$}\unboldmath{}} &
          \multicolumn{3}{c|}{\textbf{Ours}} & \multicolumn{3}{c|}{\textbf{GBBS}} &
          \multicolumn{1}{@{ }c@{}}{\textbf{SM'}} & \multirow{2}{*}{\textbf{ \seq{}}} & %\multicolumn{1}{@{}c@{}|}{\textbf{ \seq{}}}
          \multicolumn{1}{c}{\cellcolorhighlight\boldmath{}\textbf{$\boldsymbol{T_{\mathit{best}}}$}\unboldmath{}} \\
          &       &
          \multicolumn{1}{c@{ }}{\textbf{par.}} & \multicolumn{1}{@{ }c@{ }}{\textbf{seq.}} & \multicolumn{1}{@{ }c@{ }|}{\textbf{spd.}} &
          \multicolumn{1}{c@{ }}{\textbf{par.}} & \multicolumn{1}{@{ }c@{ }}{\textbf{seq.}} & \multicolumn{1}{@{ }c@{ }|}{\textbf{spd.}} &
          \multicolumn{1}{c@{ }}{\textbf{}} & \multicolumn{1}{@{ }c@{ }}{\textbf{step}} & \multicolumn{1}{@{ }c@{ }|}{\textbf{}}    &
          \multicolumn{1}{c|}{\cellcolorhighlight\textbf{/ours}} &
          \multicolumn{1}{c@{ }}{\textbf{par.}} & \multicolumn{1}{@{ }c@{ }}{\textbf{seq.}} & \multicolumn{1}{@{ }c@{ }|}{\textbf{spd.}} &
          \multicolumn{1}{c@{ }}{\textbf{par.}} & \multicolumn{1}{@{ }c@{ }}{\textbf{seq.}} & \multicolumn{1}{@{ }c@{ }|}{\textbf{spd.}} &
          \multicolumn{1}{@{ }c@{}}{\textbf{14}} & \multicolumn{1}{@{}c@{}|}{\textbf{}} &
          \multicolumn{1}{c}{\cellcolorhighlight\textbf{/ours}} \\
    \toprule
    %\multicolumn{1}{r}{\multirow{4}[2]{*}{\begin{sideways}\textbf{social}\end{sideways}}}
    %\parbox[t]{\tableside}{\hspace{\goleft}\multirow{4}{*}{\rotatebox[origin=c]{90}{\bf Social}}}
    \multicolumn{1}{@{ }c@{  }}{\hspace{\goleft}\multirow{4}[2]{*}{\begin{sideways}\textbf{Social}\end{sideways}}}
          & \textbf{OK} & -     & -     & -     & -     & -     & -     & -     & -     & -     & \cellcolorhighlight-     &
          \underline{0.112} & 4.42  & 39.6   & {0.171}  & 7.04  & 41.2  & 0.304  & 11.7  & \cellcolorhighlight 1.53 \\
          & \textbf{LJ} & 0.054 & 1.44  & 26.8  & 0.118  & 1.44  & 12.1  & \underline{0.050}$^?$ & 0.141  & 2.90  & \cellcolorhighlight0.93  &
          \underline{0.121} & 4.54  & 37.6   & 0.226  & 6.00  & 26.6  & n     & 5.10  & \cellcolorhighlight 1.87 \\
          & \textbf{TW} & \underline{0.235}  & 13.2 & 56.2  & 0.387  & 19.7  & 50.9  & c     & 1.32  & 71.7  & \cellcolorhighlight1.65  &
          \underline{1.53}  & 96.9    & 63.5   & 2.84  & 173   & 61.1  & 31.5   & 177   & \cellcolorhighlight 1.86 \\
          & \textbf{FT} & -     & -     & -     & -     & -     & -     & -     & -     & -     & \cellcolorhighlight-     &
          \underline{3.44}  & 263   & 76.4  & 6.69  & 456   & 68.1  & 10.7  & 421   & \cellcolorhighlight 1.94 \\
    \midrule
    %\parbox[t]{\tableside}{\hspace{\goleft}\multirow{4}{*}{\rotatebox[origin=c]{90}{\bf Web}}}
    \multicolumn{1}{@{ }c@{  }}{\hspace{\goleft}\multirow{4}[2]{*}{\begin{sideways}\textbf{Web}\end{sideways}}}
          & \textbf{SD} & \underline{1.62}  & 85.7 & 52.9  & 5.25  & 110   & 21.0  & 4.78$^?$ & 1.86  & 104   & \cellcolorhighlight 1.15  &
          \underline{3.35}  & 257   & 76.7   & 6.42  & 395   & 61.6  & n     & 315   & \cellcolorhighlight 1.92 \\
          & \textbf{CW} & \underline{15.8}  & 982 & 62.2  & 40.4  & 1,166 & 28.9  & n     & n     & 589   & \cellcolorhighlight2.56  &
          \underline{24.2}  & 1279  & 52.9   & 52.1  & 2515  & 48.3  & n     & 2532  & \cellcolorhighlight 2.16 \\
          & \textbf{HL14} & \underline{21.6}  & 1,487 & 68.8  & 67.3  & 2,041 & 30.3  & n     & n     & 620   & \cellcolorhighlight3.12  &
          \underline{34.7} & 1558  & 44.9   & 94.8$^?$     & 2181$^?$     & 23.0     & n     & 3914  & \cellcolorhighlight 2.73 \\
          & \textbf{HL12} & \underline{100}   & 7,699 & 76.9  & 361   & 7,022 & 19.5  & n     & n     & 1822  & \cellcolorhighlight 3.61  &
          \underline{91.4}      &   4236    &  46.4     & n     & n     & n     & n     & o     & \cellcolorhighlight - \\
    \midrule
    %\multicolumn{1}{r}{\multirow{2}[2]{*}{\begin{sideways}\textbf{Road}\end{sideways}}}
    %\parbox[t]{\tableside}{\hspace{\goleft}\multirow{2}{*}{\rotatebox[origin=c]{90}{\bf Road}}}
    \multicolumn{1}{@{ }c@{  }}{\hspace{\goleft}\multirow{2}[2]{*}{\begin{sideways}\textbf{Road}\end{sideways}}}
          & \textbf{USA} & -     & -     & -     & -     & -     & -     & -     & -     & -     & \cellcolorhighlight -     &
          \underline{0.373} & 17.4  & 46.7  & \textcolorhighlight{5.26}  & 45.3  & 8.60   & \textcolorhighlight{17.7}  & 3.13  & \cellcolorhighlight 8.40 \\
          & \textbf{GE} & -     & -     & -     & -     & -     & -     & -     & -     & -     & \cellcolorhighlight -     &
          \underline{0.285} & 20.1  & 70.6   & 2.13  & 28.6  & 13.5  & \textcolorhighlight{5.48}  & 5.22  & \cellcolorhighlight 7.48 \\
    \midrule    %\multicolumn{1}{r}{\multirow{8}[2]{*}{\begin{sideways}\textbf{KNN}\end{sideways}}}
    %\parbox[t]{\tableside}{\hspace{\goleft}\multirow{8}{*}{\rotatebox[origin=c]{90}{\bf KNN}}}
    \multicolumn{1}{@{ }c@{  }}{\hspace{\goleft}\multirow{8}[2]{*}{\begin{sideways}\textbf{KNN}\end{sideways}}}
          & \textbf{HH5} & \underline{0.253} & 3.19  & 12.6  & \textcolorhighlight{3.95}  & 3.51  & 0.89   & \textcolorhighlight{0.791}  & \textcolorhighlight{2.21}     & 0.449  & \cellcolorhighlight 1.78  &
          \underline{0.082} & 2.18  & 26.6  & 0.54  & 2.74  & 5.10   & n     & 0.81  & \cellcolorhighlight 6.57 \\
          & \textbf{CH5} & \textcolorhighlight{0.646}  & 5.54  & 8.58   & \textcolorhighlight{8.39}  & 5.84  & 0.70   & \textcolorhighlight{2.15}  & \textcolorhighlight{17.6}  & \underline{0.427}  & \cellcolorhighlight 0.66  &
          \underline{0.136} & 3.32  & 24.5  & \textcolorhighlight{1.68}  & 10.8  & 6.46   & n     & 1.03  & \cellcolorhighlight 7.59 \\
          & \textbf{GL2} & \underline{0.630}  & 41.2  & 65.4  & 3.00  & 82.4  & 27.5  & \textcolorhighlight{t}     & \textcolorhighlight{8.36}     & 3.39  & \cellcolorhighlight 4.76  &
          \underline{0.453} & 19.2  & 42.4   & 2.47  & 53.4  & 21.7  & n     & 4.07  & \cellcolorhighlight 5.45 \\
          & \textbf{GL5} & \underline{0.909}  & 47.6  & 52.3  & \textcolorhighlight{10.5}  & 91.0  & 8.69   & \textcolorhighlight{t}     & \textcolorhighlight{19.1}     & 4.83  & \cellcolorhighlight 5.32  &
          \underline{0.521} & 28.0  & 53.9   & 3.54  & 60.0  & 16.9  & n     & 7.55  & \cellcolorhighlight 6.80 \\
          & \textbf{GL10} & \underline{1.33}  & 56.5  & 42.4  & \textcolorhighlight{12.3}  & 76.5  & 6.24   & \textcolorhighlight{35.2}  & 7.14     & 9.30  & \cellcolorhighlight 5.37  &
          \underline{0.706} & 48.7  & 68.9   & 2.24  & 57.4  & 25.6  & n     & 16.6  & \cellcolorhighlight 3.17 \\
          & \textbf{GL15} & \underline{1.83}  & 67.3  & 36.8  & \textcolorhighlight{13.7}  & 84.5  & 6.15   & \textcolorhighlight{29.4}  & 10.6     & 11.3  & \cellcolorhighlight 5.78  &
          \underline{0.801} & 57.3  & 71.5   & 2.39  & 79.6  & 33.3  & n     & 22.5  & \cellcolorhighlight 2.98 \\
          & \textbf{GL20} & \underline{2.09}  & 76.5  & 36.6  & \textcolorhighlight{14.5}  & 96.6  & 6.68   & \textcolorhighlight{27.3}  & 12.3     & 13.3  & \cellcolorhighlight 5.90  &
          \underline{0.927} & 64.5  & 69.5   & 2.38  & 86.9  & 36.5  & n     & 27.8  & \cellcolorhighlight 2.57 \\
          & \textbf{COS5} & \underline{3.09}  & 232   & 75.0  & 12.0  & 367   & 30.7  & \textcolorhighlight{t}     & 57.4     & 189   & \cellcolorhighlight 3.88  &
          \underline{8.98} & 693   & 77.2  & 24.3  & 1018  & 41.9  & n     & 252   & \cellcolorhighlight 2.71 \\
    \midrule    %\multicolumn{1}{c}{\multirow{6}[2]{*}{\begin{sideways}\textbf{Synthetic}\end{sideways}}}
    \multicolumn{1}{@{ }c@{  }}{\hspace{\goleft}\multirow{6}[2]{*}{\begin{sideways}\textbf{Synthetic}\end{sideways}}}
    %\parbox[t]{\tableside}{\hspace{\goleft}\multirow{6}{*}{\rotatebox[origin=c]{90}{\bf Synthetic}}}
          & \textbf{SQR} & \underline{0.520}  & 24.2  & 46.5  & 11.1  & 28.5  & 2.57   & 4.45$^?$ & 12.6  & 15.5  & \cellcolorhighlight 8.55  &
          \underline{1.55} & 65.3  & 42.1  & \textcolorhighlight{t}     & t     & t     & n     & 11.8  & \cellcolorhighlight 7.61 \\
          & \textbf{REC} & \underline{0.099}  & 2.06  & 20.9  & \textcolorhighlight{3.82}  & 2.14  & 0.56   & 1.19$^?$ & \textcolorhighlight{5.24}  & 1.57  & \cellcolorhighlight 12.1  &
          \underline{0.17} & 5.85  & 33.8   & \textcolorhighlight{4.00}  & 18.0  & 4.50   & n     & 1.20  & \cellcolorhighlight 6.93 \\
          & \textbf{SQR'} & \underline{1.66}  & 122   & 73.6  & 4.76  & 243   & 51.0  & \textcolorhighlight{26.4$^?$} & 3.19     & 6.90  & \cellcolorhighlight 1.92  &
          \underline{1.43} & 58.8  & 41.2  & \textcolorhighlight{17.5}  & 203   & 11.6  & n     & 12.1  & \cellcolorhighlight 8.50 \\
          & \textbf{REC'} & \underline{0.168}  & 9.83  & 58.6  & \textcolorhighlight{1.00}  & 18.7  & 18.8  & \textcolorhighlight{0.851$^?$} & \textcolorhighlight{0.645}     & 0.60  & \cellcolorhighlight 3.55  &
          \underline{0.168} & 5.59  & 33.2   & \textcolorhighlight{2.91}  & 16.9  & 5.81   & n     & 1.16  & \cellcolorhighlight 6.89 \\
          & \textbf{Chn7} & -     & -     & -     & -     & -     & -     & -     & -     & -     & \cellcolorhighlight -     &
          \underline{0.282} & 23.7  & 84.1   & \textcolorhighlight{83.1}   & 48.8  & 0.59   & t     & 5.94  & \cellcolorhighlight 21.0 \\
          & \textbf{Chn8} & -     & -     & -     & -     & -     & -     & -     & -     & -     & \cellcolorhighlight -     &
          \underline{3.48} & 294   & 84.5  & \textcolorhighlight{960}     & 766     & 0.80     & t     & 65.5  & \cellcolorhighlight 18.8 \\
    \bottomrule
    \end{tabular}%%
    \vspace{-1.5em}
  \caption{\small\textbf{Running time (in seconds) and speedup of all implementations on SCC and BCC.}\label{tab:sccbcc}
  $T_{\mathit{best}}/\mathit{ours}$ (highlighted) is the \textbf{fastest time of the other implementations $/$ our time}.
  We note that in many cases the fastest baseline is standard sequential algorithm.
  The fastest runtime for each graph is underlined.
  %We verify correctness by comparing the number of SCCs and BCCs with the sequential algorithm.
  %``MS'' $=$ Multi-step algorithm in~\cite{}. ``iSpan'' $=$ iSpan algorithm in~\cite{}. ``SM'14''$=$ the \emph{faster} of BFS-BiCC and color-BiCC algorithm in~\cite{}.
  ``Std seq.'' $=$ classic sequential SCC~\cite{tarjan1972depth} and BCC~\cite{hopcroft1973algorithm} algorithms, respectively.
  Details about the baselines are introduced in \cref{sec:exp}.
  Red numbers are parallel running times \emph{slower than sequential algorithms}.
  ``par.'' $=$ parallel running time (on 192 threads). ``seq.''$=$ sequential running time (on 1 thread). ``spd.''$=$ self-speedup.
  ``?''$=$ different answer from other implementations.
  ``-''$=$ not applicable. ``t''$=$ timeout (more than 5 hours). ``c''$=$ crash. ``n''$=$ no support. ``o''$=$ out of memory.
}
\end{table*}%




==> tables/graphtable-full-old.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet2'
\begin{table*}[hp]
% \begin{flushleft}
% {\large
% \vspace{-1em}
% % \textbf{To reviewers:}

% % Our appendices start from here.
% % We understand that the reviewers are not obligated to read the appendix, and all our main results are presented in the main text.
% % We put the appendices with the main file in case reviewers want to check some information in the appendix, which can be found more conveniently using hyperlinks.
% % %We believe that the figures and tables are useful supplemental materials for understanding the performance of our algorithms and existing ones, but all major claims are justified in the main text.
% % We will provide a full version of this paper containing the appendices online.

% % As figures and tables are usually easy to read, we put our additional figures and tables first.
% % }
% \end{flushleft}

\vspace{.1in}

  \centering
  \small
    % \begin{tabular}{lrrrrrrrrrr}
    \begin{tabular}{lrrrrrrrr}
           \multicolumn{1}{c}{} & \multicolumn{1}{c}{$\boldsymbol{n}$} & \multicolumn{1}{c}{$\boldsymbol{m}$} & \multicolumn{1}{c}{$\boldsymbol{diameter}$} & \multicolumn{1}{c}{$\boldsymbol{|\mathit{SCC}_1|}$} & \multicolumn{1}{c}{$\boldsymbol{|\mathit{SCC}_1|/n}$} & \multicolumn{1}{c}{\textbf{\#SCC}} & \multicolumn{1}{c}{\textbf{Notes}} \\
           \midrule
          \multicolumn{9}{c}{\bf Social Networks}\\\midrule
    %\multicolumn{1}{r}{\multirow{4}[0]{*}{\begin{sideways}\textbf{social}\end{sideways}}}
           \textbf{LJ} & 4,847,571  & 68,993,773     & 16     & 3,828,682 & 78.98\% & 971,232 & \multicolumn{1}{l}{soc-LiveJournal1~\cite{backstrom2006group}} \\
           \textbf{TW} & 41,652,231 & 1,468,365,182 & *65     & 33,479,734 & 80.38\% & 8,044,729 &Twitter~\cite{kwak2010twitter} \\
          \midrule
    %\multicolumn{1}{r}{\multirow{4}[0]{*}{\begin{sideways}\textbf{Web}\end{sideways}}}
           \multicolumn{9}{c}{\bf Web Graphs}\\\midrule
           \textbf{SD} & 89,247,739 & 2,043,203,933 & *17  & 47,965,727 & 53.74\% & 39,205,039 & sd\_arc~\cite{webgraph} \\
           \textbf{CW} & 978,408,098 & 42,574,107,469 &  *16   & 774,373,029 & 79.15\% & 135,223,661 & ClueWeb~\cite{webgraph} \\
           \textbf{HL14} & 1,724,573,718 & 64,422,807,961 &  *793  & 320,754,363 & 18.60\% & 1,290,550,195 & Hyperlink14~\cite{webgraph} \\
           \textbf{HL12} & 3,563,602,789 & 128,736,914,167  & *5,275  & 1,827,543,757 & 51.28\% & 1,279,696,892 & Hyperlink12~\cite{webgraph} \\
          \midrule
    %\multicolumn{1}{r}{\multirow{8}[0]{*}{\begin{sideways}\textbf{KNN}\end{sideways}}}
           \multicolumn{9}{c}{\bf KNN Graphs}\\\midrule
           \textbf{HH5} & 2,049,280 & 10,246,400 & *980  & 257,914 & 12.59\% & 94,010 & \multicolumn{1}{l}{Household ~\cite{uciml,wang2021geograph}, $k=5$} \\
           \textbf{CH5} & 4,208,261 & 21,041,305 &  *4,550  & 497,331 & 11.82\% & 248,227 & \multicolumn{1}{r}{29.7M} & CHEM~\cite{fonollosa2015reservoir,wang2021geograph}, $k=5$  \\
           \textbf{GL2} & 24,876,978 & 49,753,956 & *13  & 5,368 & 0.02\% & 9,705,931 & \multicolumn{1}{l}{GeoLife~\cite{geolife,wang2021geograph}, $k=2$} \\
           \textbf{GL5} & 24,876,978 & 124,384,890  & *4,622 & 860,403 & 3.46\% & 3,198,626 & \multicolumn{1}{l}{GeoLife~\cite{geolife,wang2021geograph}, $k=5$} \\
           \textbf{GL10} & 24,876,978 & 248,769,780  & *3,172  & 3,042,330 & 12.23\% & 326,811 & \multicolumn{1}{l}{GeoLife~\cite{geolife,wang2021geograph}, $k=10$} \\
           \textbf{GL15} & 24,876,978 & 373,154,670  & *5,491  & 3,239,156 & 13.02\% & 187,646 & \multicolumn{1}{l}{GeoLife~\cite{geolife,wang2021geograph}, $k=15$} \\
           \textbf{GL20} & 24,876,978 & 497,539,560 & *5,275 & 3,336,963 & 13.41\% & 128,021 & \multicolumn{1}{l}{GeoLife~\cite{geolife,wang2021geograph}, $k=20$} \\
           \textbf{COS5} & 321,065,547 & 1,605,327,735 & *1,148 &301,413,787 & 93.88\% & 2,273,690 & \multicolumn{1}{l}{Cosmo50~\cite{cosmo50,wang2021geograph}, $k=5$} \\
          \midrule
    %\multicolumn{1}{c}{\multirow{6}[1]{*}{\begin{sideways}\textbf{Synthetic}\end{sideways}}}
           \multicolumn{9}{c}{\bf Synthetic Graphs}\\\midrule
           \textbf{SQR} & 100,000,000 & 300,000,074 & *10,002  & 99,101,606 & 99.10\% & 829,495 & \multicolumn{1}{l}{2D grid $10^4\times10^4$} \\
           \textbf{REC} & 10,000,000 & 30,000,778  & *5,946  & 9,890,647 & 98.91\% & 101,059 & \multicolumn{1}{l}{2D grid $10^3\times10^4$} \\
           \textbf{SQR'} & 100,000,000 & 120,299,012 & *14   & 58    & 0.00\% & 78,052,793 & \multicolumn{1}{l}{Sampled 2D grid $10^4\times10^4$} \\
           \textbf{REC'} & 10,000,000 & 12,031,898 & *80   & 42    & 0.00\% & 7,819,050 & \multicolumn{1}{l}{Sampled 2D grid $10^3\times10^4$} \\
    \bottomrule
    \end{tabular}
    \vspace{-1em}
    \caption{\label{tab:graphfull} \textbf{The full information of all tested graphs in this paper.} $n=$ number of vertices. $m_{\mathit{dir}}=$ number of directed edges. $m_{\mathit{sym}}=$ number of undirected edges (each edge is counted twice in both directions. For directed graphs, this is obtained by symmetrizing the graph). $D_{\mathit{dir}}=$ diameter of the directed graph. $D_{\mathit{sym}}=$ diameter of the undirected/symmetrized graph. \#CC $=$ number of connected components. $|\mathit{SCC}_1|=$ largest strongly connected component (SCC) size. $|\mathit{SCC}_1|/n=$ ratio of the largest SCC. \#SCC $=$ number of SCCs. \#BCC $=$ number of biconnected components. ``-'' $=$ does not apply.
    Diameter numbers with note ``*'' are estimated values, which is a lower bound of the actual values.
    The citations and description of these graphs can be found in Table \ref{tab:graphinfo}.
    }
    %\vspace{-2em}
    \includegraphics[width=\textwidth]{figures/speedup2.pdf}
  %\caption{Speedup\label{fig:speedup}}
  \vspace{-.5in}
\captionof{figure}{\small \textbf{Self-relative speedup for our algorithms and the algorithms in GBBS.}  Much of our performance improvement comes from better parallelism. \label{fig:speedup}}
\end{table*}%


==> tables/graphtable.tex <==
\newcommand{\tableside}{1.5mm}
\begin{table}[htbp]
  \centering
  \small
    \begin{tabular}{rlrrrl}
    \multicolumn{1}{r}{} & \multicolumn{1}{r}{} & \multicolumn{1}{c}{$\boldsymbol{n}$} & \multicolumn{1}{c}{$\boldsymbol{m_{D}}$} & \multicolumn{1}{c}{$\boldsymbol{m_{U}}$}  & \bf Notes \\
    \midrule
    %\multicolumn{1}{r|}{\multirow{4}[2]{*}{\begin{sideways}\textbf{social}\end{sideways}}}
    \parbox[t]{\tableside}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\bf Social}}}
    %\parbox[t]{\tableside}{\hspace{-1em}\multirow{4}{*}{\rotatebox[origin=c]{90}{\bf Social}}}
    & \textbf{OK} & 3.07M & -  & 234M     & com-orkut~\cite{yang2015defining} (undirected) \\
          & \textbf{LJ} & 4.85M & 69.0M & \multicolumn{1}{r}{85.7M} & \multicolumn{1}{l}{soc-LiveJournal1~\cite{backstrom2006group}} \\
          & \textbf{TW} & 41.7M & 1.47B & \multicolumn{1}{r}{2.41B} & Twitter~\cite{kwak2010twitter} \\
          & \textbf{FT} & 65.6M & - & 3.61B     & Friendster~\cite{yang2015defining} (undirected) \\
    \midrule
    %\multicolumn{1}{r|}{\multirow{4}[2]{*}{\begin{sideways}\textbf{Web}\end{sideways}}}
    \parbox[t]{\tableside}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\bf Web}}}
    & \textbf{SD} & 89.2M & 2.04B & \multicolumn{1}{r}{3.88B} & sd\_arc~\cite{webgraph} \\
          & \textbf{CW} & 978M  & 42.6B & \multicolumn{1}{r}{74.74B} & ClueWeb~\cite{webgraph} \\
          & \textbf{HL14} & 1.72B & 64.4B & \multicolumn{1}{r}{124B} & Hyperlink14~\cite{webgraph} \\
          & \textbf{HL12} & 3.56B & 129B  & 226B     & Hyperlink12~\cite{webgraph} \\
    \midrule
    %\multicolumn{1}{r|}{\multirow{2}[2]{*}{\begin{sideways}\textbf{Road}\end{sideways}}}
    \parbox[t]{\tableside}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\bf Road}}}
    & \textbf{USA} & 23.9M & - & 57.7M     & RoadUSA~\cite{roadgraph} (undirected) \\
          & \textbf{GE} & 12.3M & - & 32.3M     & Germany~\cite{roadgraph} (undirected) \\
    \midrule
    %\multicolumn{1}{r|}{\multirow{8}[2]{*}{\begin{sideways}\textbf{KNN}\end{sideways}}}
    \parbox[t]{\tableside}{\multirow{8}{*}{\rotatebox[origin=c]{90}{\bf KNN}}}
    & \textbf{HH5} & 2.05M & 10.2M & \multicolumn{1}{r}{13.0M} & \multicolumn{1}{l}{Household ~\cite{uciml,wang2021geograph}, $k=5$} \\
          & \textbf{CH5} & 4.21M & 21.0M & \multicolumn{1}{r}{29.7M} & CHEM~\cite{fonollosa2015reservoir,wang2021geograph}, $k=5$ \\
          & \textbf{GL2} & 24.9M & 49.8M & \multicolumn{1}{r}{65.4M} & \multicolumn{1}{l}{GeoLife~\cite{geolife,wang2021geograph}, $k=2$} \\
          & \textbf{GL5} & 24.9M & 124M  & \multicolumn{1}{r}{157M} & \multicolumn{1}{l}{GeoLife~\cite{geolife,wang2021geograph}, $k=5$} \\
          & \textbf{GL10} & 24.9M & 249M  & \multicolumn{1}{r}{305M} & \multicolumn{1}{l}{GeoLife~\cite{geolife,wang2021geograph}, $k=10$} \\
          & \textbf{GL15} & 24.9M & 373M  & \multicolumn{1}{r}{453M} & \multicolumn{1}{l}{GeoLife~\cite{geolife,wang2021geograph}, $k=15$} \\
          & \textbf{GL20} & 24.9M & 498M  & \multicolumn{1}{r}{602M} & \multicolumn{1}{l}{GeoLife~\cite{geolife,wang2021geograph}, $k=20$} \\
          & \textbf{COS5} & 321M  & 1.61B & \multicolumn{1}{r}{1.96B} & \multicolumn{1}{l}{Cosmo50~\cite{cosmo50,wang2021geograph}, $k=5$} \\
    \midrule
    %\multicolumn{1}{r|}{\multirow{5}[2]{*}{\begin{sideways}\textbf{Synthetic}\end{sideways}}}
    \parbox[t]{\tableside}{\multirow{5}{*}{\rotatebox[origin=c]{90}{\bf Synthetic}}}
    & \textbf{SQR} & 100M  & 300M  & \multicolumn{1}{r}{400M} & \multicolumn{1}{l}{2D grid $10^4\times10^4$} \\
          & \textbf{REC} & 10M   & 30M   & \multicolumn{1}{r}{40M} & \multicolumn{1}{l}{2D grid $10^3\times10^4$} \\
          & \textbf{SQR'} & 100M  & 120M  & \multicolumn{1}{r}{204M} & \multicolumn{1}{l}{Sampled 2D grid $10^4\times10^4$} \\
          & \textbf{REC'} & 10M   & 12M   & \multicolumn{1}{r}{24M} & \multicolumn{1}{l}{Sampled 2D grid $10^3\times10^4$} \\
          & \textbf{Chn7} & 10M  & -  & 10M     & Chain of size $10^7$ (undirected) \\
          & \textbf{Chn8} & 100M  & -  & 100M     & Chain of size $10^8$ (undirected) \\
    \bottomrule
    \end{tabular}%
    \vspace{-.15in}
      \caption{\small\textbf{Graph Information.} $n=$ number of vertices. $m_D=$ number of directed edges. $m_{U}=$ number of undirected edges. For directed graphs, $m_{U}$ is obtained by symmetrizing the graph. M and B mean million and billion, respectively. Complete information of the graphs are given in \cref{tab:graphfull}.\label{tab:graph}}
  \label{tab:graphinfo}%
\end{table}%


==> tables/lssteps.tex <==
\hide{
\begin{table}[!h]
  \centering
  \caption{Add caption}
    \begin{tabular}{r|rr|rr}
          & \multicolumn{2}{c|}{\textbf{Forward}} & \multicolumn{2}{c}{\textbf{Backward}} \\
          & \multicolumn{1}{c}{\textbf{plain}} & \multicolumn{1}{c|}{\textbf{+LS}} & \multicolumn{1}{c}{\textbf{plain}} & \multicolumn{1}{c}{\textbf{+LS}} \\
    \midrule
    \multicolumn{1}{l|}{$0^*$} & 10001 & 111   & 10001 & 112 \\
    1     & 1     & 1     & 1     & 1 \\
    2     & 2     & 1     & 3     & 1 \\
    3     & 3     & 1     & 2     & 1 \\
    4     & 4     & 1     & 3     & 1 \\
    5     & 3     & 1     & 3     & 1 \\
    6     & 3     & 1     & 3     & 1 \\
    7     & 3     & 1     & 5     & 1 \\
    8     & 4     & 1     & 4     & 1 \\
    9     & 4     & 1     & 4     & 1 \\
    10    & 6     & 1     & 6     & 1 \\
    11    & 6     & 1     & 5     & 1 \\
    12    & 5     & 1     & 4     & 1 \\
    13    & 5     & 1     & 5     & 1 \\
    14    & 8     & 1     & 7     & 1 \\
    15    & 8     & 1     & 9     & 1 \\
    16    & 8     & 1     & 6     & 1 \\
    17    & 11    & 1     & 6     & 1 \\
    18    & 6     & 1     & 8     & 1 \\
    19    & 9     & 1     & 8     & 1 \\
    20    & 7     & 1     & 8     & 1 \\
    21    & 8     & 1     & 7     & 1 \\
    22    & 8     & 1     & 8     & 1 \\
    23    & 8     & 1     & 8     & 1 \\
    24    & 8     & 1     & 7     & 1 \\
    25    & 7     & 1     & 8     & 1 \\
    26    & 6     & 1     & 6     & 1 \\
    27    & 5     & 1     & 4     & 1 \\
    \end{tabular}%
  \label{tab:addlabel}%
\end{table}%
}

\hide{
% Table generated by Excel2LaTeX from sheet 'Sheet9'
\begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{r|rr|rr}
          & \multicolumn{2}{c|}{\textbf{Forward}} & \multicolumn{2}{c}{\textbf{Backward}} \\
          & \multicolumn{1}{c}{\textbf{plain}} & \multicolumn{1}{c|}{\textbf{w/ LS}} & \multicolumn{1}{c}{\textbf{plain}} & \multicolumn{1}{c}{\textbf{w/ LS}} \\
    \midrule
    \multicolumn{1}{c|}{SCC1} & 92    & 1     & 88    & 1 \\
    1     & 3     & 1     & 7     & 1 \\
    2     & 5     & 1     & 7     & 1 \\
    3     & 166   & 3     & 187   & 3 \\
    4     & 1622  & 44    & 1745  & 38 \\
    5     & 2609  & 49    & 2512  & 42 \\
    6     & 35    & 1     & 32    & 1 \\
    7     & 287   & 4     & 200   & 2 \\
    8     & 165   & 4     & 320   & 4 \\
    9     & 5206  & 27    & 5308  & 28 \\
    10    & 1626  & 19    & 4070  & 22 \\
    11    & 513   & 8     & 512   & 8 \\
    12    & 5337  & 24    & 5334  & 24 \\
    13    & 1070  & 9     & 1125  & 6 \\
    14    & 3236  & 18    & 4541  & 26 \\
    15    & 12059 & 54    & 12053 & 54 \\
    16    & 3678  & 20    & 3672  & 20 \\
    17    & 2817  & 15    & 2758  & 14 \\
    18    & 1944  & 12    & 1954  & 11 \\
    19    & 2654  & 14    & 2030  & 11 \\
    20    & 1855  & 11    & 1483  & 10 \\
    21    & 2225  & 12    & 2197  & 11 \\
    22    & 1503  & 10    & 1520  & 10 \\
    23    & 883   & 5     & 860   & 5 \\
    24    & 573   & 6     & 622   & 6 \\
    25    & 377   & 4     & 408   & 4 \\
    26    & 343   & 3     & 321   & 4 \\
    27    & 258   & 3     & 254   & 3 \\
    28    & 193   & 3     & 165   & 3 \\
    29    & 131   & 3     & 134   & 4 \\
    30    & 109   & 3     & 112   & 3 \\
    31    & 108   & 3     & 103   & 3 \\
    32    & 64    & 3     & 85    & 3 \\
    33    & 45    & 3     & 51    & 3 \\
    34    & 32    & 3     & 34    & 3 \\
    35    & 22    & 3     & 23    & 3 \\
    36    & 16    & 2     & 17    & 3 \\
    37    & 12    & 2     & 12    & 2 \\
    38    & 9     & 2     & 8     & 2 \\
    39    & 5     & 2     & 6     & 2 \\
    40    & 2     & 1     & 2     & 1 \\
    \end{tabular}%
  \label{tab:addlabel}%
\end{table}%
}
%\newpage
\begin{table*}[p]
\includegraphics[width=\textwidth]{figures/subrounds.pdf}
  %\caption{Speedup\label{fig:speedup}}
   \vspace{-.2in}
% \captionof{figure}{\small \textbf{Self-relative speedup for our algorithms and the algorithms in GBBS.}  Much of our performance improvement comes from better parallelism. \label{fig:speedup}}
\captionof{figure}{\textbf{Number of rounds with and without local search for each batch.} The number $k$ in the title of each figure means that on that graph, using local search reduces the number of rounds in reachability searches by $k$ times on average. \label{fig:SCC-rounds}}

\begin{minipage}[!t]{\columnwidth}
  %\centering
  \small
  %\begin{flushleft}
    \begin{tabular}{@{}r|r@{ }r@{ }|r@{ }r@{ }|r@{ }r@{ }|r@{ }r@{ }}
    \multicolumn{1}{r}{} & \multicolumn{4}{c}{\textbf{GL5}} & \multicolumn{4}{c}{\textbf{SQR}} \\
          & \multicolumn{2}{c|}{\textbf{Forward}} & \multicolumn{2}{c|}{\textbf{Backward}} & \multicolumn{2}{c|}{\textbf{Forward}} & \multicolumn{2}{c}{\textbf{Backward}} \\
          & \multicolumn{1}{c}{\textbf{plain}} & \multicolumn{1}{@{ }c@{ }|}{\textbf{+LS}} & \multicolumn{1}{c}{\textbf{plain}} & \multicolumn{1}{@{ }c@{ }|}{\textbf{+LS}} & \multicolumn{1}{c}{\textbf{plain}} & \multicolumn{1}{@{ }c@{ }|}{\textbf{+LS}} & \multicolumn{1}{c}{\textbf{plain}} & \multicolumn{1}{@{ }c@{ }}{\textbf{+LS}} \\
    \midrule
    \multicolumn{1}{@{}c|}{$0^*$} & 92    & 1     & 88    & 1     & 10001 & 111   & 10001 & 112 \\
    1 &3 &1 &7 &1 &1 &1 &1 &1 \\
    2 &5 &1 &7 &1 &2 &1 &3 &1 \\
    3 &166 &3 &187 &3 &3 &1 &2 &1 \\
    4 &1622 &44 &1745 &36 &4 &1 &3 &1 \\
    5 &2609 &51 &2512 &42 &3 &1 &3 &1 \\
    6 &35 &1 &32 &1 &3 &1 &3 &1 \\
    7 &287 &4 &200 &2 &3 &1 &5 &1 \\
    8 &165 &4 &320 &4 &4 &1 &4 &1 \\
    9 &5206 &27 &5308 &28 &4 &1 &4 &1 \\
    10 &1626 &19 &4070 &22 &6 &1 &6 &1 \\
    11 &513 &8 &512 &8 &6 &1 &5 &1 \\
    12 &5337 &24 &5334 &24 &5 &1 &4 &1 \\
    13 &1070 &9 &1125 &6 &5 &1 &5 &1 \\
    14 &3236 &18 &4541 &26 &8 &1 &7 &1 \\
    15 &12059 &54 &12053 &54 &8 &1 &9 &1 \\
    16 &3678 &20 &3672 &20 &8 &1 &6 &1 \\
    17 &2817 &15 &2758 &15 &11 &1 &6 &1 \\
    18 &1945 &12 &1954 &11 &6 &1 &8 &1 \\
    19 &2654 &14 &2030 &11 &9 &1 &8 &1 \\
    20 &1855 &11 &1481 &10 &7 &1 &8 &1 \\
    21 &2225 &12 &2197 &11 &8 &1 &7 &1 \\
    22 &1504 &10 &1518 &10 &8 &1 &8 &1 \\
    23 &883 &5 &860 &5 &8 &1 &8 &1 \\
    24 &573 &6 &623 &5 &8 &1 &7 &1 \\
    25 &376 &4 &408 &4 &7 &1 &7 &1 \\
    26 &343 &3 &321 &3 &6 &1 &6 &1 \\
    27 &258 &3 &254 &3 &4 &1 &4 &1 \\
    28 &193 &3 &165 &3 & & & & \\
    29 &131 &3 &134 &3 & & & & \\
    30 &112 &3 &112 &3 & & & & \\
    31 &108 &3 &103 &3 & & & & \\
    32 &64 &4 &84 &3 & & & & \\
    33 &45 &3 &51 &3 & & & & \\
    34 &33 &3 &32 &3 & & & & \\
    35 &22 &2 &24 &3 & & & & \\
    36 &17 &2 &17 &3 & & & & \\
    37 &12 &2 &12 &2 & & & & \\
    38 &9 &1 &8 &2 & & & & \\
    39 &6 &2 &6 &2 & & & & \\
    40 &2 &1 &2 &1 & & & & \\
    \end{tabular}%
  \captionof{table}{\small\textbf{Number of rounds needed in SCC, with or without local search, on GL5 and SQR graphs.}
  ``Plain''$=$ using regular BFS-based search. ``+LS''$=$ using local searches.
  ``$0^{*}$''$=$ single-reachability search to find the first SCC (first row).
  The rest of steps are steps in prefix doubling, which use multi-source searches.
  \label{tab:sccsteps}}%
  %\end{flushleft}
  \end{minipage}\hfill
  \begin{minipage}[!t]{\columnwidth}%\vspace{0pt}
  %\begin{flushright}
    \input{tables/CCLLtable}\vspace{2in}
  %\end{flushright}
  \end{minipage}
\end{table*}%
\newpage



==> tables/scc-rounds.tex <==
\begin{figure}[th]
  \includegraphics[width=\columnwidth]{figures/scripts/subrounds_oneColumn.pdf}
  % \vspace{-.2in}
  \caption{\small\revision{\small \textbf{Number of rounds with and without local search for each batch.}} All settings are the same as \cref{tab:graphfull}.
  %On \knn graphs, the average numbers of rounds can be reduced by 20--180x using local queues with size at most 2^9.
  Each data point $(x,y)$ means that in one reachability search, $y$ rounds are needed using local search, and $x$ rounds are needed without local search.
  %The number $k$ in the title of each figure means that on that graph, using local search reduces the number of rounds in reachability searches by $k$ times on average.
  The number ``avg'' for each graph is the average number of $k=y/x$ for all data points, which means, on average, using local search reduces the number of rounds needed by a factor of $k$.
  \label{fig:SCC-rounds} }
  %\vspace{-.2in}
\end{figure}


==> total_break.tex <==


\hide{
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{figures/BCC_breakdown_total.pdf}
  \caption{BCC Breakdown For All Graphs}\label{fig:BCC_Total_Break}
\end{figure*}
} 
